Adaptivity Gaps for the Stochastic Boolean Function Evaluation Problem

We consider the Stochastic Boolean Function Evaluation (SBFE) problem where the task is to efficiently evaluate a known Boolean function $f$ on an unknown bit string $x$ of length $n$. We determine $f(x)$ by sequentially testing the variables of $x$, each of which is associated with a cost of testing and an independent probability of being true. If a strategy for solving the problem is adaptive in the sense that its next test can depend on the outcomes of previous tests, it has lower expected cost but may take up to exponential space to store. In contrast, a non-adaptive strategy may have higher expected cost but can be stored in linear space and benefit from parallel resources. The adaptivity gap, the ratio between the expected cost of the optimal non-adaptive and adaptive strategies, is a measure of the benefit of adaptivity. We present lower bounds on the adaptivity gap for the SBFE problem for popular classes of Boolean functions, including read-once DNF formulas, read-once formulas, and general DNFs. Our bounds range from $\Omega(\log n)$ to $\Omega(n/\log n)$, contrasting with recent $O(1)$ gaps shown for symmetric functions and linear threshold functions.

==> Adaptivity Gap/sections/draft.tex <==
\paragraph{Papers with adaptivity gap techniques:}
\begin{itemize}
    \item \href{https://link.springer.com/article/10.1007/s10107-015-0927-9}
    {On the Adaptivity Gap of Stochastic Orienteering (Bansal, Nagarjan)}:
    Uses binary tree construction to get lower bound.
    \item
    \href{https://arxiv.org/pdf/1608.00673.pdf}
    {Adaptivity Gaps for Stochastic Probing:Submodular and XOS Functions (Gupta, Nagarajan, Singla)}:Improves on results of Asadpour et al. and others.  Gives constant-factor adaptivity gap for maximizing monotone submodular fn subject to a very general class of constraints, called prefix-closed constraints (including matroid constraints, knapsack constraints, cardinality constraints). 
    They survey previous techniques including e.g.: use LP relaxations to lower bound optimal cost of adaptive strategy, use multilinear extension of submodular fns -- and then try to find a non-adaptive strategy that is close to this lower bound.  Instead, they take an adaptive strategy and show that you can get a non-adaptive strategy from it with low expected cost (not much more than the adaptive strategy) by randomly choosing a root-leaf path as your non-adaptive strategy.  And this shows that a non-adaptive strategy with low expected cost exists. 
    \item \href{https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.142.9979&rep=rep1&type=pdf}{Stochastic Submodular Maximization. (Asadpour, Nazerzadeh)}: using Poisson clock
    \item \href{https://theory.stanford.edu/~jvondrak/data/knapsack_focs.pdf}{Approximating the Stochastic Knapsack Problem: The Benefit of Adaptivity (Dean, Goemans, Vondrak)}
    \item \href{https://researcher.watson.ibm.com/researcher/files/us-jvondrak/stoch_cover.pdf}{Stochastic covering and adaptivity. (Goemans, Vondrak)}
    \item \href{https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.481.772&rep=rep1&type=pdf}{Adaptivity and Approximation for Stochastic Packing Problems (Dean, Goemans, Vondrak)}:
    Uses construction to get lower bound.
    \item
    \href{https://arxiv.org/abs/1504.02146}{Discrete Stochastic Submodular Maximization: Adaptive vs. Non-adaptive vs. Offline (Hellerstein, Kletenik, Lin)}: Starts with an adaptive tree and proves that you can collapse it into a single path (non-adaptive strategy) in such a way that the resulting expected cost isn't too much bigger than the expected cost of the original tree.  The bound obtained depends on the $p_i$'s.  
\end{itemize}

\teal{Upper bound of adaptivity gap is number of variables
from increasing greedy cost non-adaptive strategy.}

\teal{Say unit cost}

\teal{Add what we know about symmetric functions.}

\teal{$O(k)$ upper bound on adaptivity gap where $k$
is number of terms in a read once DNF.
Adaptive strategy can either keep querying the same term
or move to another.
We know what term it will query in each term
(highest probability of resolving / cost), so if 
we round robin between terms then we get $O(k)$
times adaptive.}

\lnf{
The adaptivity gap was first introduced in the study of stochastic knapsack problem by Dean et al.~\cite{DBLP:conf/focs/DeanGV04}, and in that particular problem they showed the adaptivity gap is 8, and later Bhalgat~\cite{bhalgat2+} improved it to $2+\varepsilon$. Dean et al.~\cite{DBLP:conf/soda/DeanGV05} generalized it to the stochastic packing problem, in which they allow the knapsack constraints to be multidimensional. Gupta et al.~\cite{DBLP:conf/soda/GuptaNS16} study the stochastic probing problem and gave a $O(\log n)$ adaptivity gap. Later Gupta et al.~\cite{DBLP:conf/soda/GuptaNS17} improved it to 3 and Bradac et al.~\cite{DBLP:conf/approx/Bradac0Z19} improved it to 2, which is close to the lower bound $\frac{e}{e-1}$ given by Asadpour et al.~\cite{DBLP:conf/wine/AsadpourNS08}. Fu et al.~\cite{DBLP:conf/icalp/FuLX18} gave a PTAS for a class of stochastic dynamic programs, which include the probing problem and variants of the stochastic knapsack problem. Although the adaptivity gaps for stochastic maximization problems are well studied, there has been little progress on stochastic minimization problems. Goemans et al.~\cite{DBLP:conf/latin/GoemansV06} study the stochastic covering problem, and they showed if the items can be used repeatedly, the adaptivity gap is $\Theta(\log d)$ where d is the size of target set to be covered. They also pointed out the adaptivity gap can be arbitrarily large if the items can be used only once. Recently Ghuge et al.~\cite{Ghuge21} showed constant the adaptivity gap for the stochastic score classification problem, which was previously introduced by Gkenosis et al.~\cite{gkenosisetal18}. All those results make us wondering what is the adaptivity gap for the SBFE problem.
}


%\section{Monotone DNF}
%
%\begin{theorem}
%There is a monotone DNF
%with $N$ terms and $N + 2\log_2 N$ variables
%where the optimal non-adaptive
%strategy has expected cost $\Omega(N^{.32})$
%times the optimal adaptive strategy.
%\end{theorem}
%
%\begin{proof}
%
%\item \paragraph{Construction}
%
%The monotone DNF construction is equivalent to the DNF
%construction except that we replace $\overline{x}_i$ with
%a new independent variable $x_i'$.
%Additionally, each $x$-variable is still 1 with probability 1/2
%but each $y$-variable is 1 with probability 1.
%\teal{We'll eventually talk about extending to the
%uniform setting so our lower bound result is stronger.}\lnf{I agree, and I'll work on this tonight.}
%
%\item \paragraph{Adaptive Expected Cost}
%
%We argue that the optimal adaptive strategy tests the $x$
%variables before testing any of the $y$-variables since each
%$x$-variable gives information about strictly more
%terms than any $y$-variable.
%Without loss of generality, we test in order of increasing index.
%If $x_i=1$, we continue to $x_{i+1}$.
%If $x_i=0$, we test $x_i'$ since there's a $(1-p)^2$ probability
%we will immediately find a 0-certificate.
%
%If we test all of the $x$-variables without finding a 0-certificate,
%then we know exactly which terms have only 1's and with a single
%additional test we will have a 1-certificate.
%
%Using this optimal strategy, 
%we can generate the following decision tree:
%Let $c(n)$ denote the expected cost of the optimal decision tree with $n$ of $x_i$ (also $n$ of $x_i'$ and $2^n$ of $y_i$),
%we can write the following:
%\begin{align*}
%    c(n) = p\cdot c(n-1) + (1-p)\cdot (p\cdot c(n-1)+1) + 1
%\end{align*}
%
%Since $p=0.5$, we have
%\begin{align*}
%    c(n) &= 0.5\cdot c(n-1) + 0.5\cdot (0.5\cdot c(n-1)+1) + 1\\
%    &=0.75\cdot c(n-1)+1.5\\
%    c(n)-6 &= 0.75\cdot (c(n-1) -6)
%\end{align*}
%
%Hence, $c(n)$ converges to 6 when $n\rightarrow \infty$
%and the expected cost of the optimal adaptive strategy
%is constant.
%
%\item \paragraph{Non-Adaptive Expected Cost}
%
%We do not know what the optimal non-adaptive strategy
%is but we argue that it tests all the $x$-variables
%before any of the $y$-variables for the same reason
%as the optimal adaptive strategy.
%If there is a 0-certificate then the non-adaptive strategy
%also has constant expectation.
%If there is a 1-certificate then the non-adaptive strategy
%will test all of the $x$-variables and then
%need to find a $y$-variable in a term with only 1's.
%The high-level idea is that finding such a $y$-variable
%is difficult for the non-adaptive strategy.
%
%Formally,
%we argue that the expected cost of finding a 1-certificate
%is very high.
%In order to lower bound this expectation, we partition
%assignments with 1-certificates based on the number of
%pairs $t$ where $x_i=x_i'=1$ for $i \in [n]$.
%The probability that there are $t$ pairs is
%$\binom{n}{t} (1/4)^t (1/2)^{n-t}$ since there's a $1/4$ probability
%pair $i$ has $x_i=x_i'=1$, a $1/2$ probability either
%$x_i=1$ or $x_i'=1$, and $\binom{n}{t}$ ways to choose
%these pairs.
%
%The expected cost of a non-adaptive strategy finding a
%term with a 1-certificate is
%$(2^n+n)/2^{t+1} \geq 2^{n-t-1}$ by the following argument.
%
%Say that an assignment to the $x_i, x_i'$ pairs is a `t-assignment' if
%\begin{enumerate}
%    \item for $t$ of the $x_i,x_i'$ pairs, $x_i=x_i'=1$, and
%    \item for the other $n-t$ pairs, exactly one 
%    of $x_i$ and $x_i'$ is equal to 1.
%\end{enumerate}
%
%Consider any non-adaptive ordering of the $y$-variables.
%Without loss of generality, we relabel the variables so
%the non-adaptive ordering is
%$y_1,y_2,...,y_{N}$ with corresponding terms
%$t_1,\ldots,t_{N}$.
%
%Let $A$ be a random $t$-assignment, chosen uniformly
%from all $t$-assignments.
%%(as before, we assume
%%that all $y$-variables are set to 1 in this assignment).
%Let $c(A)$ denote the number of tests on $y$-variables
%that are performed on $A$ according to a non-adaptive strategy.
%We want to show a lower bound on the expected value of $c(A)$.
%
%The value of $c(A)$
%is the unique index $i$ such that $A$ 
%does not satisfy the terms associated 
%with $y_1,..,y_{i-1}$,
%but $A$ does satisfy the term associated with $y_i$.
%
%Let $Z = \binom{n}{t}$. There are $Z*2^{n-t}$ total $t$-assignments.
%For any particular $i$, term $t_i$ is satisfied by
%exactly $Z$ many of these $t$-assignments.
%Thus the probability that $A$ satisfies a particular term $t_i$
%is $Z / (Z*2^{n-t})$ = $1 / (2^{n-t})$.
%It follows from a Union Bound that for any particular $i$,
%the probability that $A$ satisfies $t_1$ or $t_2$ or ... or $t_i$
%is less than $i / 2^{n-t}$.
%
%Therefore,
%\begin{align*}
%    \Pr(c(A) > i ) \geq 1 - \frac{i}{2^{n-t}}.
%\end{align*}
%
%Now consider a random variable $X$ that takes values
%in $[2^{n-t}]$ with uniform probability. 
%For each $i$ in the support of $X$,
%$\Pr(X > i) = 1 - i / 2^{n-t}$.
%Since $X$ is equally likely to take any value between 1 and
%$2^{n-t}$, its expected value is $2^{n-t}/2$.
%Observe that
%$\Pr(c(A) > i) \geq \Pr(X > i)$
%for all $i \in [n]$.
%Therefore the expected value of $c(A)$ is
%lower bounded by the expected value of $X$ which is $2^{n-t}/2$.
%
%Then the expected cost of any non-adaptive strategy
%finding a 1-certificate is at least
%\begin{align*}
%    \frac{1}{2} \sum_{t=0}^n 
%    \binom{n}{t} (1/4)^t (1/2)^{n-t} (2^{n-1})
%    = \frac{1}{2} \sum_{t=0}^n 
%    \binom{n}{t} (1/4)^t = (1+1/4)^n
%\end{align*}
%where the last equality follows from the observation that
%the sum is an ordinary generating function of the binomial
%sequence.
%Using $n = \log_2 N$,
%we get that the expected cost is
%$N^{\log_2 5/4} \approx N^{.32}$.
%
%\end{proof}

%Although we don't know what's exactly the optimal non-adaptive strategy, 
%we can lower-bound it. 
%We use conditional expectation here. 
%Let $\E{\OPT}$ denote the optimal non-adaptive strategy, then we let $\E{\OPT\mid g=i}$ to denote the expected cost to evaluate the function when there are $i$ terms being 1 and $p_i$ to be the probability that there are $i$ terms being 1.
%Hence, we have the following
%\begin{align}
%    \E{\OPT} = \sum_{i=0}^{2^n}\E{\OPT\mid g=i}\cdot p_i \label{eq:1}
%\end{align}
%
%We first take a look at $p_i$. Notice that
%\begin{itemize}
%    \item When $i=1$, it means \textit{only one of each $\{x_i, x_i'\}$ is 1}. Hence, $p_1=\frac{1}{2}^n$.
%    \item When $i=2$, it means \textit{only one of each $\{x_i, x_i'\}$ is 1, except there exist one pair that both of $\{x_i, x_i'\}$ are 1}. Hence, $p_2=(\frac{1}{2})^{n-1}\cdot\frac{1}{4}\cdot {n\choose 1}$.
%    \item When $i=3$, $p_3=0$ since it's only possible to have $2^{k}$ terms to be one, where $k\in\{0,1,\dots,n\}$.
%\end{itemize}
%
%Hence we can rewrite part of (\ref{eq:1}) to the following:
%\begin{align}
%    \E{\OPT \mid g\geq 2}\cdot p_{g\geq 2} &= \sum_{i=1}^{t}\E{\OPT\mid g=2^t}\cdot p_{2^t}\notag\\
%    &=\sum_{t=1}^{n}\E{\OPT\mid g=2^t}\cdot (\frac{1}{2})^{n-t}\cdot\frac{1}{2}^{2t}\cdot {n \choose t}\label{eq:2}
%\end{align}
%
%Next we deal with $\E{\OPT\mid g=i}$.
%\begin{itemize}
%    \item When $i=1$, $\E{\OPT\mid g=i}=\frac{1}{2}\cdot 2^n$
%    \item When $i=2$, $\E{\OPT\mid g=i}=\frac{1}{2}\cdot 2^{n-1}$
%    \item When $i=4$, $\E{\OPT\mid g=i}=\frac{1}{2}\cdot 2^{n-2}$
%\end{itemize}
%
%Hence, $\E{\OPT\mid g=i}=2^{n-i-1}$. Apply this to (\ref{eq:2}) we have the following:
%\begin{align}
%    (\ref{eq:2})=\sum_{t=1}^n 2^{n-t-1}\cdot (\frac{1}{2})^{n-t}\cdot\frac{1}{2}^{2t}\cdot {n \choose t} := \sum_{t=1}^n h(t)\label{eq:3}
%\end{align}
%
%When $t=1$,
%\begin{align*}
%    h(1)=2^{n-2-n+1-2}\cdot n = (\frac{1}{2})^3\cdot n
%\end{align*}
%
%Hence, $\E{\OPT} = \Omega(n)=\Omega(\log N)$.
%

\section{Notes for 7/14}
\begin{itemize}
    \item The non-monotone DNF also works for polynomial-size decision tree.
    \item open problems
    \begin{itemize}
        \item is the adaptivity gap for arbitrary Boolean function $\Omega(n)$?\\
        \lnf{for arbitrary cost, I think yes. By replacing the unit-cost of $y_i$ with a large cost will yields adaptivity gap of $\Omega(n)$}
        \item Is the adaptivity gap for arbitrary monotone functions
less than it is for arbitrary non-monotone Boolean functions?
Can you show e.g. that the gap is no more than O(sqrt(N))
for the uniform distribution and unit costs?
    \end{itemize}
\end{itemize}

\section{Symmetric functions}
\begin{itemize}
    \item Upper bound of symmetric function with unit cost is 2. \lnf{actually 4, according to the previous error}
    \item Upper bound of symmetric function with arbitrary cost is something close to 8 (CHECK THIS). 
\end{itemize}

==> Adaptivity Gap/sections/intro.tex <==
\section{Introduction}

We consider the question of determining adaptivity gaps for the Stochastic Boolean Function Evaluation (SBFE) problem, for different classes of Boolean formulas.
% Fix a positive integer $n$. 
% In the SBFE problem for a Boolean function $f:\{0,1\}^n \rightarrow \{0,1\} $, 
In an SBFE problem,
we are given a (representation of a) Boolean function 
$f:\{0,1\}^n \rightarrow \{0,1\}$,
a positive cost vector $c=[c_1, \ldots, c_n]$,
and a probability vector $p=[p_1, \ldots, p_n]$.
The problem is to determine the value $f(x)$
on an initially unknown random input $x \in \{0,1\}^n$.
The value of each $x_i$ can only be determined by performing a test, which incurs a cost of $c_i$.  Each $x_i$ is equal to 1 (is true) with independent probability $p_i$.
Tests are performed sequentially and
continue until $f(x)$ can be determined.
We say $f(x)$ is determined by a set of tests
if $f(x) = f(x')$ for all $x' \in \{0,1\}^n$ 
such that $x'_i=x_i$ for every $i$ in the set of tests. 

For example, if $f(x) = x_1 \vee \ldots \vee x_n$  then testing continues until a test is performed on some $x_i$ such that $x_i=1$ at which point we know $f(x)=1$,
or until all $n$ tests have been performed 
with outcome $x_i=0$ for each $x_i$ so we know $f(x)=0$.
The problem is to determine the order to perform tests that minimizes
the total expected cost of the tests. 

We will call a testing order a strategy which we can think of
as a decision tree for evaluating $f$.
A strategy can be {\em adaptive},
meaning that the choice of the next test $x_i$ can depend 
on the outcome of previous tests. 
In some practical settings, however, it is desirable 
to consider only {\em non-adaptive} strategies.
Non-adaptive strategies often take up less space than adaptive strategies, and they may be able to be evaluated more quickly if tests can be performed in parallel~\cite{DBLP:conf/soda/GuptaNS17}, such as in the problem of detecting network faults~\cite{harvey2007non} or in group testing for viruses, such as the coronavirus~\cite{liva2021optimum}.
A non-adaptive testing strategy is a permutation of the tests
where
testing continues in the order specified by the permutation 
until the value of $f(x)$ can be determined from the outcomes of the tests performed so far.
A non-adaptive strategy also corresponds to a decision tree
where all non-leaf nodes on the same level contain the same test $x_i$.

The {\em adaptivity gap} measures how much benefit 
can be obtained by using an adaptive strategy.
Consider a class $F$ of $n$-variable functions $f:\{0,1\}^n \rightarrow \{0,1\}$.
Let $\OPT_\N(f,c,p)$ be the expected evaluation cost of the optimal
non-adaptive strategy on function $f$ under costs $c$ and probabilities $p$.
Similarly, $\OPT_\A(f,c,p)$ is the expected evaluation cost of
the optimal adaptive strategy on $f$ under $c$ and $p$.
The adaptivity gap of the function class $F$ is
\begin{align*}
    \max_{f \in F}
    \sup_{c,p}
    \frac{\OPT_\N(f,c,p)}{\OPT_\A(f,c,p)}.
\end{align*}
%If we draw $x$ from the product 
%For
%input assignment $x \in \{0,1\}^n$,
%define $\cost_c(f, x, S)$ to be the total cost of the tests performed
%in applying strategy $S$ to $x$, with respect to the costs in $c$.
%Define $\cost_{c,p}(f, S):=E_{x \sim D_p}[\cost_c(f,x,S)]$,
%where $D_p$ is the the product distribution defined by $p$.
%Define $\OPT_{\A}(f,c,p)$
%to be the minimum value of
%$\cost_{c,p}(f, S)$ over all adaptive strategies $S$ for evaluating $f$
%and $OPT_{\N}(f,c,p)$ to be the analogous quantity for non-adaptive strategies.
%The adaptivity gap of the SBFE problem for the class of functions (or Boolean formulas) $F$ 
%is the function $\alpha(n) := \max_{(f,c,p) \in {\cal I}_n} \OPT_\N(f,c,p)/\OPT_\A(f,c,p)$,
%where ${\cal I}_n$ is the set of all triples $(f,c,p)$ 
%such that $f \in F$ is a function of $n$
%variables, and
%and $c$ and $p$ are cost and probability vectors of length $n$.
% Define $\cost_\A^{c,p}(f):= \min_{S \in \A} \cost(f, S)
%\textnormal{ and }
%\cost_\N(f):= \min_{S \in \N} \cost(f, S).$$  
% We will drop the superscript ${c,p}$ when dealing with unit
% costs and the uniform distribution.
%So, for example, $\cost(f,S) = \cost^{c,p}(f,S)$ for $c=[1,\ldots,1]$ and $p=[1/2,\ldots,1/2]$.
%$$\cost(f, S):= \E_{x \sim D}[\cost(f,x,S)].$$
%We represent an instance of the SBFE problem as a triple
%$I=(f,p,c)$, where 
%$f:\{0,1\}^n \rightarrow \{0,1\}$ is the function to evaluate,  $p = [p_1, \ldots, p_n]$ is the vector of probabilities, and $c=[c_1, \ldots, c_n]$ is the vector of costs.  For $I=(f,p,c)$
%let $\cost_\N(I)$ be the minimum expected cost 
%of evaluating $f$ over non-adaptive strategies
%and $\cost_\A(I)$ be the minimum expected cost
%of evaluating $f$ over adaptive strategies, where the expectation is with respect to $p$ and $c$.
%Let $F$ be a class of Boolean functions, and for $n > 0$, let $I_n$ denote the wet of instances $I=(f,p,c)$ 
%where $f:\{0,1\}^n \rightarrow \{0,1\}$ and $f \in F$.
%The adaptivity gap of the SBFE problem for the class $F$ 
%is the function $\alpha(n) := \max_{I \in I_n} \cost_\N(I)/\cost_\A(I)$.

The SBFE problem for a class of Boolean 
formulas $F$ restricts the evaluated $f$ to be a member of $F$.
In this paper we prove bounds on the adaptivity gaps for the SBFE problem on 
read-once DNF formulas,
DNF formulas, and read-once formulas.
(See Section~\ref{preliminaries} for definitions.)
A summary of our results can be found in Table~\ref{table:results}.
%As indicated in the table, many of the lower bound results still apply in restricted cases of the problem, such as unit costs, the uniform distribution (i.e., each $p_i = 1/2$), or equal probabilities (all $p_i$'s are equal).
%Note our lower bound results are stated in the most restricted case
%(e.g., unit costs, uniform probabilities where $p_i=1/2$,
%or equal probabilities where $p_i=p_j$ for all $i,j$)
%because they apply by definition
%to more general forms of the problem.
% Note many of our results are lower bounds, they can be easily extended to more general cases in which some of the restrictions, like unit costs, can be removed.

%The lower bounds for unit cost or uniform distribution versions of the SBFE problem also apply, by definition, to the standard SBFE problem with arbitrary
%costs and probabilities. The same is not true for upper bounds.
%All of our lower bounds apply even to the case of unit costs $c_i=1$ unless otherwise indicated. 

All the 
% lower 
bounds in the table have a dependence on $n$, meaning that none of the listed SBFE problems has a constant adaptivity gap.  This contrasts with recent work of Ghuge et al.~\cite{Ghuge21}, which shows that the adaptivity gaps for the SBFE problem for symmetric Boolean functions and linear threshold functions are $O(1)$. 

For any SBFE problem, the non-adaptive strategy of testing the $x_i$ in increasing order of $c_i$ has an expected cost that is within a factor of $n$ of the optimal adaptive strategy~\cite{DBLP:conf/stoc/KaplanKM05}.  Thus $n$ is an upper bound on the adaptivity gap for all SBFE problems.

\begin{table}[ht]
\centering
\caption{A summary of our results. We also prove an $O(\sqrt{n})$
upper bound for tribes formulas i.e., read-once DNFs with unit costs
where every term has the same number of variables.
We say all probabilities are equal if $p_1 = p_2 = \ldots = p_n$.}
\label{table:results}
{\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|l|l|}
 \hline
 \textbf{Formula Class} &  \textbf{Adaptivity Gap} \\
\hline
\multirow{3}{*}{Read-once DNF}
&  $\Theta(\log n)$ for unit costs, uniform distribution\\
\cline{2-2}
 &  $\Omega(\sqrt{n})$ for unit costs\\
\cline{2-2}
& $\Omega(n^{1-\epsilon}/\log n)$ for uniform distribution\\
\hline
Read-once & $\Omega(\epsilon^3 n^{1-2\epsilon/\ln(2)})$ for unit costs, equal probabilities\\
\hline
\multirow{2}{*}{DNF}
& $\Omega(n/\log n)$ for unit costs, uniform distribution\\
\cline{2-2}
& $\Theta(n)$ for uniform distribution \\
\hline
\end{tabular}
}
\end{table}




%\begin{table}[h]
%\centering
%\caption{A summary of our results.
%*Indicates the upper bound only applies for
%read-once DNFs where every term has the same
%number of variables.}
%\label{table:results}
%{\renewcommand{\arraystretch}{1.2}
%\begin{tabular}{|l|l|l|l|}
% \hline
% \textbf{Formula Class} & %\textbf{Costs} 
% & \textbf{Probabilities} & %\textbf{Adaptivity Gap} \\
%\hline
%Read-once DNF & Unit & Uniform & $O(\log n)$ and $\Omega(\log n)$ \\
%\hline 
%Read-once DNF & Unit & Arbitrary & $O(\sqrt{n})$* and $\Omega(\sqrt{n})$ \\
%\hline
%Read-once DNF & Arbitrary & Uniform & $\Omega(n/\log n)$ \\
%\hline
%Read-once Formula & Unit & Constant & $\Omega(\epsilon^3 n^{1-2\epsilon/\ln(2)})$ \\
%\hline
%Non-Monotone DNF & Unit & Uniform & $\Omega(n/\log n)$ \\
%\hline
%\end{tabular}
%}
%\end{table}

\textbf{Outline:} We present our results on formula classes
in increasing order of generality.
In Section \ref{sec:read-once}, we warm up with a variety of
results on read-once DNF formulas in different settings.
In Section \ref{sec:formula},
we prove our main technical result for read-once formulas,
drawing on branching process identities and concentration 
inequalities.
In Section \ref{sec:dnf}, we prove our most general results
on DNF formulas (the bounds also apply to the restricted
class of DNF formulas with a linear number of terms).
Note that we state our lower bound results in the most 
restricted context because they of course apply to more
general settings.
Due to space constraints, we defer some proofs to 
Appendix $\ref{app:delayed}$.

\subsection{Connection to $st$-connectivity in uncertain networks}

Our result for read-once formulas has implications for a problem
of determining $st$-connectivity in an uncertain network,
studied by Fu et al.~\cite{DBLP:journals/ton/FuFXPWL17}.
The input is a multi-graph with a 
source node $s$ and a destination node $t$.
Each edge corresponds to a variable $x_i$ indicating whether it is usable,
which is true with probability $p_i$.
Testing the usability of edge $i$ costs $c_i$.
The $st$-connectivity function for the multi-graph is true if and only if
there is a path of usable edges from $s$ to $t$.
The problem is to find a strategy to evaluate
the $st$-connectivity function that has minimum expected cost.

%Our result for read-once formulas has implications for a problem 
%of determining $st$-connectivity in an uncertain network,
%studied by Fu et al.~\cite{DBLP:journals/ton/FuFXPWL17}.
%The input is a multi-graph with a source node $s$ and a destination node $t$.
%Each edge $i$ corresponds to a variable $x_i$ that can be tested
%for a cost of $c_i$ and realizes to usable or unusable with probability $p_i$.
%The $st$-connectivity function is true if and only if
%there is a path of usable edges from $s$ to $t$.

%The input to the problem is a multi-graph $G$ with source node $s$ and destination node $t$, and for each edge $e$, a cost $c_e$ and a probability $p_e$. 
%Each edge $e$ in the graph is either ``usable'' or ``unusable''.
%Edge $e$ is usable with independent probability $p_e$.
%The only way to determine whether edge $e$ is usable is to perform a test with cost $c_e$.
%The problem is to determine the order in which to perform tests 
%so as to minimize the expected cost of determining whether 
%there is a path of usable edges from $s$ to $t$.
%This is an SBFE problem for a Boolean function $f$, defined by $G$, $s$, and $t$, whose input variables correspond to the edges in $G$,
%and whose output is true if and only if there is a path from $s$ to $t$
%whose associated edge variables are all set to true.
%We call such a function $f$ an {\em $st$-connectivity function}.
%Thus the problem of determining $st$-connectivity in an uncertain network is equivalent to the SBFE problem for $st$-connectivity functions $f$.

The $st$-connectivity function associated with a multi-graph can be represented 
by a read-once formula if and only if the multi-graph is a two-terminal series-parallel graph.
This type of graph has two distinguished nodes, $s$ and $t$, and is formed by recursively combining disjoint series-parallel graphs either in series, or in parallel (see \cite{eppstein1992parallel} for the precise definitions).\footnote{The term {\it series-parallel circuits} (systems) refers to a set of parallel circuits that are connected in series (see, e.g.,~\cite{el1986optimal,wiki:Series_and_parallel_circuits}).
%\lisa{Naifeng, fill in a citation or two?  Maybe to series-parallel circuits?}\lnf{I don't know if there's a good reference for series-parallel circuits (it looks like basic knowledge in papers mentioning it), so I put a wikipedia page as reference for now}  
Viewed as graphs,
they correspond to the subset of two-terminal series-parallel graphs whose $st$-connectivity functions correspond to read-once CNF formulas.  We note that Kowshik used the term ``series-parallel graph'' in a non-standard way to refer only to this subset; Fu et al.\, in citing Kowshik, used the term the same way~\cite{kowshik2011information,DBLP:journals/ton/FuFXPWL17}.}
Fu et al.\ performed experiments with both adaptive and non-adaptive strategies for this problem, comparing their performance, but did not prove theoretical adaptivity gap bounds.
Since the $st$-connectivity function on a series-parallel graph
is a read-once formula,
our lower bound on the adaptivity gap for read-once formulas
applies to the problem of $st$-connectivity. 

\subsection{Related work}
It is well-known that the SBFE problem for the Boolean OR function given by $f(x) = x_1 \vee \ldots \vee x_n$ has a simple solution:
test the variables $x_i$ in increasing order of the ratio $c_i/p_i$ until  a test reveals a variable set to true, or until all variables are tested and found to be false (cf.~\cite{Unluyurt04}). This strategy is non-adaptive, meaning that the SBFE problem for the Boolean OR function has an adaptivity gap of 1. That is, there is no benefit to adaptivity. 

Gkenosis et al.~\cite{gkenosisetal18} introduced the Stochastic Score Classification problem, which generalizes the SBFE problem for both symmetric Boolean functions and for linear threshold functions.  
Ghuge et al.~\cite{Ghuge21} showed that the Stochastic Score Classification problem has an adaptivity gap of $O(1)$.
In the unit-cost case, Gkenosis et al.\ showed the gap is at most 4 for symmetric Boolean functions, and at most  $\phi$ (the golden ratio) for the not-all-equal function~\cite{gkenosisetal18}.

Adaptivity gaps were introduced by Dean et al.~\cite{DBLP:conf/focs/DeanGV04} in the study of the stochastic knapsack problem %\footnote{Their item values are deterministic while sizes are independent random variables with known distributions.}
which, in contrast to the SBFE problem for Boolean functions, is a maximization problem.
It has an  adaptivity gap of 4  ~\cite{DBLP:conf/focs/DeanGV04,DBLP:journals/mor/DeanGV08}.
% \devorah{they show that it's almost tight -- arbitrarily close to 4}. 
Adaptivity gaps have also been shown for other stochastic maximization problems  (e.g.,
\cite{DBLP:conf/soda/DeanGV05,DBLP:conf/soda/GuptaNS16,DBLP:conf/approx/Bradac0Z19,HKL15,DBLP:conf/wine/AsadpourNS08}).  
Notably, the problem of
maximizing a monotone submodular function with stochastic inputs, subject to any class of prefix-closed constraints,
 was shown to have an $O(1)$ adaptivity gap~\cite{DBLP:conf/soda/GuptaNS17,DBLP:conf/approx/Bradac0Z19}.

Adaptivity gaps have also been shown for stochastic covering problems, which, like SBFE, are minimization problems.
Goemans et al.~\cite{DBLP:conf/latin/GoemansV06} showed that
the adaptivity gap for the Stochastic Set Cover problem, in which each item can only be chosen once, is $\Omega(d)$ and $O(d^2)$,
where $d$ is the size of the target set to be covered.
If the items can be used repeatedly, the adaptivity gap is $\Theta(\log d)$. 

%They also showed that the adaptivity gap can be arbitrarily large if the items can only be used once.

Agarwal et al.~\cite{DBLP:conf/soda/AgarwalAK19} 
and Ghuge et al.~\cite{GhugeetalStochasticSubmod} proved bounds of $\Omega(Q)$ and $O(Q \log Q)$ respectively,
on the adaptivity gap for the more abstract Stochastic Submodular Cover Problem in which each item can only be used once. 
Applied to the special case of Stochastic Set Cover, the upper bound is $O(d \log d)$, which improves the above $O(d^2)$ bound.
They also gave bounds parameterized by the number of rounds of adaptivity allowed.
We note that, as shown by Deshpande et al.~\cite{DeshpandeGoalValue}, one approach to solving SBFE problems is to reduce them to special cases of Stochastic Submodular Cover.  However, this approach does not seem to have interesting implications for SBFE problem adaptivity gaps.
% An interesting example of an SBFE problem is 
% determining $st$-connectivity in uncertain networks, a problem defined by Fu et al.\cite{DBLP:journals/ton/FuFXPWL17} \lisa{check reference}. The input to the problem is a graph $G$ with source node $s$ and destination node $t$, and for each edge, a cost $c_e$ and a probability $p_e$. 
% Each edge $e$ in the graph is either ``usable'' or ``unusable''.
% Edge $e$ is usable with independent probability $p_e$.
% The only way to determine whether edge $e$ is usable is to perform a test with cost $c_e$.
% The problem is to determine the order in which to perform tests 
% so as to minimize the expected cost of determining whether 
% there is a path of usable edges from $s$ to $t$.
% This is an SBFE problem for a Boolean function $f$, defined by $G$, $s$, and $t$, whose input variables correspond to the edges in $G$,
% and whose output is positive if and only if there is a path from $s$ to $t$
% whose associated edge variables are all positive.
% We call such a function $f$ an $st$-connectivity function.
% Thus the problem of determining $st$-connectivity in an uncertain network is equivalent to the SBFE problem for $s$-$t$ connectivity functions $f$.

%such that the value of $f$ on an input assignment is 1 if and only if there is an $s$-$t$
%path in $G$ whose corresponding edge variables are all set to 1.




%Dean et al.~\cite{DBLP:conf/sod%a/DeanGV05} generalized the %stochastic knapsack problem to %the stochastic packing problem (in which the knapsack constraints can be multidimensional) and proved the adaptivity gap is $\Theta(\sqrt{d})$, where $d$ is the number of dimensions. 
% Gupta et al.~\cite{DBLP:conf/soda/GuptaNS16} studied the stochastic probing problem\footnote{Their goal is to maximize the expected value of picked elements, while the picked elements satisfying some constraint.} and gave a $O(\log n)$ adaptivity gap. 
%Later Gupta et al.~\cite{DBLP:conf/soda/GuptaNS17} improved it to 3 and Bradac et al.~\cite{DBLP:conf/approx/Bradac0Z19} improved it to 2, which is close to the lower bound $\frac{e}{e-1}$ given by Asadpour et al.~\cite{DBLP:conf/wine/AsadpourNS08}. 
%Fu et al.~\cite{DBLP:conf/icalp/FuLX18} gave a polynomial time approximation scheme (PTAS) for a class of stochastic dynamic programs, which include the probing problem and variants of the stochastic knapsack problem. 
%This paper concerns adaptivity gaps for the SBFE problem, which is a stochastic minimization problem. Previously, Ghuge et al.\ showed an $O(1)$ adaptivity gap for the Stochastic Score Classifcation Problem; this immediately implies an $O(1)$ adaptivity gap for the SBFE problem for symmetric Boolean functions and for linear threshold functions~\cite{Ghuge21}.



%There has been less work on adaptivity gaps for stochastic minimization problems. Goemans et al.~\cite{DBLP:conf/latin/GoemansV06} studied the stochastic covering problem, and  showed if the items can be used repeatedly, the adaptivity gap is $\Theta(\log d)$ where $d$ is the size of target set to be covered. They also observed that the adaptivity gap can be arbitrarily large if the items can only be used once. Recently Ghuge et al.~\cite{Ghuge21} showed a constant adaptivity gap for the stochastic score classification problem, which was previously introduced by Gkenosis et al.~\cite{gkenosisetal18}.
%Together, previous results for the adaptivity gaps of 
%stochastic optimization problems naturally suggest
%the study of adaptivity gaps in the context of SBFE.


% Our result for read-once formulas has implications for a problem of determining $st$-connectivity in an uncertain network, studied by Fu et al.~\cite{DBLP:journals/ton/FuFXPWL17}. Consider a network (multi-graph) with designated nodes $s$ and $t$. Suppose each edge $e$ in the network has an associated probability $p_e$, which is the probability that the edge is usable. This probability is independent of the probability that other edges are usable.
% The $p_e$ values are given, and we need to determine whether or not there is a path of intact edges from $s$ to $t$. Testing the usability of edge $e$ incurs a given cost $c_e$. The problem is to determine the order in which to test the edges so as to minimize expected testing cost. This is actually an SBFE problem, with the $x_i$ corresponding to the edges in the graph. \lnf{Would it be helpful to say, the $st$-connectivity problem in an uncertain network corresponds to the SBFE problem for DNF? As each possible s-t path is a term, and each edge on that path is a variable in that term}\lisa{Every Boolean fn can be represented by a DNF. Because we define $f$ here, it immediately follows that there is a DNF associated with $f$. So every SBFE problem is an SBFE problem for DNF -- sort of. I say sort of because if we're concerned about computational complexity, then we need to take into account how the Boolean function is represented, which determines the size of the input. But in this paper, we do not worry about computational complexity. } Here $f(x_1, \ldots, x_n)$ is a Boolean function such that $f(x)=1$ if and only if there exists an s-t path in the multi-graph such that for each edge in the path, we have $x_i=1$ for the corresponding $x_i$. The multi-graph is two-terminal series-parallel, with terminals $s$ and $t$, if and only if the function $f$ is representable by a read-once formula~\cite{RaghavanSchach90}. (We define series-parallel graphs in Section~\ref{preliminaries}.)
% Thus the lower bound on the adaptivity gap for read-once formulas is also a lower bound on the adaptivity gap for the $st$-connectivity problem. 



% At the end of this paper, we perform experiments comparing the performance of optimal adaptive strategies and optimal non-adaptive strategies on $st$-connectivity problems, building on previous experiments of Fu et al~\cite{DBLP:journals/ton/FuFXPWL17}.
% To compute optimal adaptive strategies, we use an exponential-time dynamic programming approach which has been rediscovered by a number of different researchers, including by Fu et al.~\cite{DBLP:journals/ton/FuFXPWL17} (see also \cite{}).\lisa{Mentioned in Unyulurt survey as having been used for linear threshold function, the data mining paper on optimal decision trees, also the Raghavan and ?? paper, also Fu et al.} To compute optimal non-adaptive strategies, we develop a new dynamic programming algorithm, also taking exponential time. This algorithm can be used to generate the optimal non-adaptive strategy solving the SBFE problem for any Boolean function. 

%Because of the exponential running time of the dynamic programming algorithms, we only run these algorithms on small datasets. To explore the benefit of adaptivity on arger datasets, we compare the performance of existing and/or simple adaptive and non-adaptive heuristics. 
%Our experiments expand on previous experiments of
%Fu et al.\, who investigated different heuristics for solving the $st$-connectivity problem, some adaptive and some non-adaptive.

\subsection{Preliminaries}\label{preliminaries}
%Let $\OPT_\A(f,c,p)$ be the expected cost of %the optimal
%adaptive strategy under costs $c$ and probabilities $p$
%and $\OPT_\N(f,c,p)$ be the expected cost of the optimal
%non-adaptive strategy under costs $c$ and probabilities $p$.
%Let ${\cal F}$ be a class of Boolean functions, ${\cal C}$ be a class of cost vectors, and ${\cal P}$ be a class of probability vectors.
%Then the SBFE adaptivity gap for ${\cal F}$, ${\cal C}$, and ${\cal P}$
%is the following function of $n$:
%$\max_{f \in F_n}, \max{c \in C_n, p \in P_n} %\OPT_\N(f,c,p)/\OPT_\A(f,c,p)$
%where $F_n$, $C_n$, and $P_n$ are 
% is the set of $n$-variable functions $f \in F$.
%Our results primarily consist of adaptivity gaps
%for unit costs $c=[1,\ldots,1]$ and uniform
%probabilities $p=[1/2,\ldots,1/2]$.
%Since they are lower bounds, these results also lower bound
%the adaptivity gap for more general costs and probabilities.
%When the costs or probabilities are more general,
%the adaptivity gap includes an additional
%maximization over choices of $c$ or $p$.

Consider a Boolean function $f:\{0,1\}^n \rightarrow \{0,1\}$,
a positive cost vector $c=[c_1,\ldots,c_n]$, and probability vector
$p=[p_1,\ldots, p_n]$.
We assume $c_i > 0$ and $0 < p_i < 1$ for $i \in [n]$
where $[n]$ denotes the set $\{1, \ldots, n\}$.
Let strategy $S$ be a decision tree for evaluating $f(x)$
on an unknown input $x \in \{0,1\}^n$.
We define $\cost_c(f, x, S)$ as the total cost of the variables
tested by $S$ on input $x$ until $f(x)$ is determined.
We say $x \sim p$ if $\Pr(x)=\prod_{i:x_i=1}p_i \prod_{i:x_i=0} (1-p_i)$.
Then $\cost_{c,p}(f, S) := \E_{x \sim p}[\cost_c(f,x,S)]$
is the expected evaluation cost of strategy $S$ when
$x$ is drawn according to the product distribution induced by $p$.

For fixed $n$, let $\A$ be
the set of adaptive strategies on $n$ variables 
and $\N$ be the set of non-adaptive strategies on $n$ variables.
We are interested in the quantities 
\begin{align*}
    \OPT_\A (f,c,p) := \min_{S \in \A} \cost_{c,p}(f,S)
    \mbox{ and }
    \OPT_\N (f,c,p) := \min_{S \in \N} \cost_{c,p}(f,S).
\end{align*}
We will omit $c$ and $p$ from the notation when
the costs and probabilities are clear from context.
%An instance of an SBFE problem for a class of formulas $F$
%consists of an $n$ variable function $f \in F$, a cost vector $c$, and a probability vector
%$p$.  The adaptivity gap for the problem is then
%is $\sup_{c,p}\max_{f} \OPT_\N(f,c,p)/\OPT_\A(f,c,p)$.
A {\em (Boolean) read-once formula} is a tree, each of whose internal nodes are labeled either $\vee$ or $\wedge$. The internal nodes have two or more children. 
Each leaf is labeled with a Boolean variable $x_i \in \{x_1, \ldots, x_n\}$. The formula computes a Boolean function in the usual way.\footnote{Some definitions of a read-once formula allow negations in the internal nodes of the formula. By DeMorgan's laws, these negations can be ``pushed'' into the leaves of the formula,
resulting in a formula whose internal nodes are $\vee$ and $\wedge$, such that each variable $x_i$ appears in at most one leaf.}
A (Boolean) {\em DNF formula} is a formula of the form $T_1 \vee T_2 \vee \ldots T_m$ for some $m \geq 1$, such that each {\em term} $T_i$ is the conjunction ($\wedge$) of literals. A literal is a variable $x_i$ or a negated variable $\neg x_i$. The DNF formula is read-once if distinct terms contain disjoint sets of variables, without negations.
Read-once DNF formulas whose terms all contain the same number $w$ of literals are sometimes known as tribes formulas of width $w$ (cf.~\cite{ODonnellBook}). 

%A {\em two-terminal series-parallel graph} (TTSP) is a graph which includes two distinct, distinguished nodes $s$ and $t$ (called terminal nodes). It is defined recursively as follows. An edge is a TTSP, with endpoints $s$ and $t$. A multi-graph $G$ with terminal nodes $s$ and $t$ is a TTSP if it is produced by combining two TTSPs, $G_1$ and $G_2$, either in series, or in parallel, as follows. 
%Let $s_1$, $t_1$ and $s_2$, $t_2$, be the two terminal nodes of $G_1$ and $G_2$, respectively.
%\begin{itemize}
%  \item Parallel: $G$ is produced by merging nodes $s_1$ and $s_2$ into the single node $s$, and merging nodes $t_1$ and $t_2$ into the single node $t$. (If this results in multiple copies of the same edge, all copies are preserved.)
%  \item Series: $G$ is produced by merging nodes $t_1$ and $s_2$ into a new single node, and by setting $s = s_1$ and $t=t_2$.
%\end{itemize}
%By ``merging nodes $v$ and $w$ into the single node $z$'' we mean that whenever $v$ or $w$ appears as an endpoint of an edge, it is replaced by $z$. 
%If this results in the creation of identical edges, all copies are preserved, so that the total number of edges remains the same after the merge. 
%Given a multi-graph $G=(V,E)$ with two distinct distinguished nodes $s$ and $t$, define the {\em $st$-connectivity function} $f:\{0,1\}^{|E|} \rightarrow \{0,1\}$ of the graph as follows. Function $f$ is a Boolean function whose variables correspond to the edges of $G$. For any assignment $x \in \{0,1\}^{|E|}$, $f(x)=1$ if and only if there is an $st$ path in $G$ such that all edges in the path are set to 1 by $x$. 
%A Boolean function $f$ is expressible by a read-once formula if and only if it is the $st$-connectivity function of a two-terminal series-parallel graph~\cite{RaghavanSchach90}.

%\subsection{Literature Review}
%
%\href{https://people.cs.rutgers.edu/~sa1497/stuff/papers/stochastic_submodular-cover_2019.pdf}{Stochastic Submodular Cover with Limited Adaptivity}
%
%\href{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8057094}{Complexity vs. Optimality: Unraveling
%Source-Destination Connection in Uncertain Graphs}
%
%\begin{itemize}
%\item Read-Once DNF with Unit Costs and Uniform Probability:
%$\Omega(\log n)$ lower bound and $O(\log n)$
%\item Read-Once DNF with Unit Cost and Arbitrary Probability:
%$\Omega(\sqrt{n})$ lower bound and $O(\sqrt{n})$
%upper bound if constant length
%\item Read-Once DNF with Arbitrary Cost and 
%Uniform Probability: $\Omega(n^{1-\epsilon}/\log n)$
%\item Read-Once Formula with Unit Cost and Constant Probability: $\Omega(\epsilon^3 n^{1-2\epsilon/\ln(2)})$ lower bound
%\item DNF with Unit Costs and Uniform Probability:
%$\Omega(n/\log n)$ lower bound
%\end{itemize}
%

==> Adaptivity Gap/sections/intro_old.tex <==
\section{Introduction}

We consider the question of determining adaptivity gaps for Stochastic Boolean Function Evaluation (SBFE) problems. Fix a positive integer $n$. In the SBFE problem for a Boolean function $f:\{0,1\}^n \rightarrow \R $, we are given a (representation of) a Boolean function $f(x_1, \ldots, x_n)$ and asked to determine the value of the function on an initially unknown random input $x=(x_1,\ldots, x_n)$.  The values of the individual variables $x_i$ are independent, and for each $x_i$, we are given $p_i=P[x_i=1]$.
The value of an $x_i$ in $x$ can only be determined by performing a ``test''. Testing $x_i$ incurs a given cost $c_i$, and tests must be performed sequentially.  Testing continues until the value of $f(x)$ can be determined.  The problem is to determine the order in which to perform the tests, so as to minimize the total expected cost of the tests.  The testing order can be adaptive, meaning that the choice of the next test $x_i$ can depend on the outcome of previous tests. An adaptive test ordering, often called a ``strategy,'' corresponds to a decision tree.

An interesting example of an SBFE problem is 
determining $st$-connectivity in uncertain networks, a problem defined by Fu et al.\cite{DBLP:journals/ton/FuFXPWL17} \lisa{check reference}.  The input to the problem is a graph $G$ with source node $s$ and destination node $t$, and for each edge, a cost $c_e$ and a probability $p_e$. 
Each edge $e$ in the graph is either ``usable'' or ``unusable''.
Edge $e$ is usable with independent probability $p_e$.
The only way to determine whether edge $e$ is usable is to perform a test with cost $c_e$.
The problem is to determine the order in which to perform tests 
so as to minimize the expected cost of determining whether 
there is a path of usable edges from $s$ to $t$.
This is an SBFE problem for a Boolean function $f$, defined by $G$, $s$, and $t$, whose input variables correspond to the edges in $G$,
and whose output is positive if and only if there is a path from $s$ to $t$
whose associated edge variables are all positive.
We call such a function $f$ an $st$-connectivity function.
Thus the problem of determining $st$-connectivity in an uncertain network is equivalent to the SBFE problem for $s$-$t$ connectivity functions $f$.
%such that the value of $f$ on an input assignment is 1 if and only if there is an $s$-$t$
%path in $G$ whose corresponding edge variables are all set to 1.

In some practical settings, it is desirable to consider only ``non-adaptive'' testing strategies.  A non-adaptive testing strategy is a permutation of the tests; testing continues in the order specified by the permutation until no more testing is needed (here, until the value of $f(x)$ can be determined).
A non-adaptive strategy corresponds to an adaptive strategy whose decision tree representation has the property that all non-leaf nodes on the same level contain the same test $x_i$.

The ``adaptivity gap'' is a measure of how much benefit can be obtained from adaptivity.
Let $\cost_\N(f)$ be the minimum expected cost
of evaluating $f$ over non-adaptive strategies
and $\cost_\A(f)$ be the minimum expected cost
of evaluating $f$ over adaptive strategies.
% The adaptivity gap of the SBFE problem for $f$ is
% $\cost_\N(f)/\cost_\A(f)$.
Let $F$ be a class of Boolean functions, and let $F_n$
denote the functions in $F$ with $n$ input variables.
The adaptivity gap of the SBFE problem for the class $F$ 
is the function $g:\mathcal{N} \rightarrow \mathcal{R}$
such that for all $n \in \mathcal{N}$, 
$g(n) = \max_{f \in F} \cost_\N(f)/\cost_\A(f)$.

It is well-known that the SBFE problem for the Boolean OR function given by $f(x_1, \ldots, x_n) = x_1 \vee \ldots \vee x_n$ has a simple solution:  
test the variables $x_i$ in increasing order of the ratio $c_i/p_i$ until finding some variable is positive, or all variables are found to be negative. This strategy is non-adaptive, meaning that the SBFE problem for the Boolean OR function has an adaptivity gap of 1.  That is, there is no benefit to adaptivity.  

It is also known that, for arbitrary Boolean functions, the non-adaptive strategy of testing the $x_i$ in increasing order of $c_i$ has an expected cost that is within a factor of $n$ of the optimal adaptive strategy~\cite{DBLP:conf/stoc/KaplanKM05}\lisa{add cite}. Thus the adaptivity gap for the SBFE problem on any class of Boolean functions is somewhere between 1 and $n$.  

In this paper we prove adaptivity gaps for the SBFE problem on (the class of functions) associated with three well-studied classes of Boolean formulas:

\begin{table}[]
\centering
\caption{A summary of our results.
*Indicates the upper bound only applies for
read-once DNFs where every term has the same
number of variables.}
{\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|l|l|l|l|}
 \hline
 \textbf{Formula Class} & \textbf{Costs} 
 & \textbf{Probabilities} & \textbf{Adaptivity Gap} \\
\hline
Read-once DNF & Unit & Uniform & $O(\log n)$ and $\Omega(\log n)$ \\
\hline 
Read-once DNF & Unit & Arbitrary & $O(\sqrt{n})$* and $\Omega(\sqrt{n})$ \\
\hline
Read-once DNF & Arbitrary & Uniform & $\Omega(n/\log n)$ \\
\hline
Read-once Formula & Unit & Constant & $\Omega(\epsilon^3 n^{1-2\epsilon/\ln(2)})$ \\
\hline
Non-Monotone DNF & Unit & Uniform & $\Omega(n/\log n)$ \\
\hline
\end{tabular}
}
\bigskip
\end{table}

\bigskip
\begin{tabular}{c|c}

\end{tabular}

An $st$-connectivity function associated with a graph $G$ can be represented by a read-once formula if and only if the graph $G$ is series-parallel~\cite{RaghavanSchach90}.
Thus our lower bound on the adaptivity gap for read-once formulas also applies to the problem of $st$-connectivity in uncertain networks.  \lisa{say something about Fu et al.'s experimental adaptivity gap observations?}

\bigskip
All of our lower bounds apply even to the case of unit costs $c_i=1$. These non-constant gaps contrast 
with the constant-factor adaptivity gaps shown previously for
the SBFE problem for symmetric functions and for linear threshold functions~\cite{gkenosisetal18}.
%
%
%.  Grammel et al.\ showed an upper bound of 4 on the additivity gap for the class of symmetric functions in the unit-cost case (and smaller gaps for certain subclasses of the symmetric functions)~\cite{}. Ghuge et al.\ showed an upper bound of $8+\epsilon$, on the adaptivity gap for the class of symmetric functions and the class of linear threshold functions, under arbitrary costs~\cite{}.  


 \lnf{shall we also mention the constant adaptivity gap for many other stochastic discrete optimization problems? e.g. stochastic knapsack, probing, covering, etc.}\lisa{I think it's enough to contrast with the previous SBFE results, especially now that I've been able to add the recent Ghuge et al. results.}

Our result for read-once formulas has implications for a problem of determining $st$-connectivity in an uncertain network, studied by Fu et al.~\cite{DBLP:journals/ton/FuFXPWL17}.  Consider a network (multi-graph) with designated nodes $s$ and $t$.  Suppose each edge $e$ in the network has an associated probability $p_e$, which is the probability that the edge is usable. This probability is independent of the probability that other edges are usable.
The $p_e$ values are given, and we need to determine whether or not there is a path of intact edges from $s$ to $t$.  Testing the usability of edge $e$ incurs a given cost $c_e$.  The problem is to determine the order in which to test the edges so as to minimize expected testing cost.  This is actually an SBFE problem, with the $x_i$ corresponding to the edges in the graph. \lnf{Would it be helpful to say, the $st$-connectivity problem in an uncertain network corresponds to the SBFE problem for DNF? As each possible s-t path is a term, and each edge on that path is a variable in that term}\lisa{Every Boolean fn can be represented by a DNF.  Because we define $f$ here, it immediately follows that there is a DNF associated with $f$.  So every SBFE problem is an SBFE problem for DNF -- sort of.  I say sort of because if we're concerned about computational complexity, then we need to take into account how the Boolean function is represented, which determines the size of the input. But in this paper, we do not worry about computational complexity. }  Here $f(x_1, \ldots, x_n)$ is a Boolean function such that $f(x)=1$ if and only if there exists an s-t path in the multi-graph such that for each edge in the path, we have $x_i=1$ for the corresponding $x_i$.  The multi-graph is two-terminal series-parallel, with terminals $s$ and $t$, if and only if the function $f$ is representable by a read-once formula~\cite{RaghavanSchach90}.  (We define series-parallel graphs in Section~\ref{preliminaries}.)
Thus the lower bound on the adaptivity gap for read-once formulas is also a lower bound on the adaptivity gap for the $st$-connectivity problem.  

We note that, as originally shown by Deshpande et al.\cite{DeshpandeGoalValue}, one approach to solving SBFE problems is to reduce them to special cases of Stochastic Submodular Cover.  As shown by~\cite{DBLP:conf/soda/AgarwalAK19}, the adaptivity gap for the general Stochastic Submodular Cover problem is linear in $n$ DOUBLE-CHECK THIS.  However, their result does not imply lower bounds on the adaptivity gap for SBFE problems.  

At the end of this paper, we perform experiments comparing the performance of optimal adaptive strategies and optimal non-adaptive strategies on $st$-connectivity problems, building on previous experiments of Fu et al~\cite{DBLP:journals/ton/FuFXPWL17}.
To compute optimal adaptive strategies, we use an exponential-time dynamic programming approach which has been rediscovered by a number of different researchers, including by Fu et al.~\cite{DBLP:journals/ton/FuFXPWL17} (see also \cite{}).\lisa{Mentioned in Unyulurt survey as having been used for linear threshold function, the data mining paper on optimal decision trees, also the Raghavan and ?? paper, also Fu et al.}  To compute optimal non-adaptive strategies, we develop a new dynamic programming algorithm, also taking exponential time.  This algorithm can be used to generate the optimal non-adaptive strategy solving the SBFE problem for any Boolean function.  

%Because of the exponential running time of the dynamic programming algorithms, we only run these algorithms on small datasets.  To explore the benefit of adaptivity on arger datasets, we compare the performance of existing and/or simple adaptive and non-adaptive heuristics.  
%Our experiments expand on previous experiments of
%Fu et al.\, who investigated different heuristics for solving the $st$-connectivity problem, some adaptive and some non-adaptive.

\subsection{Preliminaries}\label{preliminaries}
Consider a Boolean function $f:\{0,1\}^n \rightarrow \R$
and a strategy $S$ for testing variables on an unknown
input $x \in \{0,1\}^n$ to determine $f(x)$.
Define $\cost(f, x, S)$ to be the cost of determining
$f(x)$ using strategy $S$.
Then let $\cost(f, S)$ be the expected
cost of evaluating $f(x)$ where $x$ is drawn
from the uniform distribution, i.e.,
$$\cost(f, S):= \E_{x \sim \{0,1\}^n}[\cost(f,x,S)].$$
Let $\A$ denote the set of all adaptive
strategies for evaluating $f$ on an input
and let $\N$ denote the set of all
non-adaptive strategies for evaluating $f$.
Then 
$$\cost_\A(f):= \min_{S \in \A} \cost(f, S)
\textnormal{ and }
\cost_\N(f):= \min_{S \in \N} \cost(f, S).$$
With this notation in hand,
the adaptivity gap of a function $f$ is 
$\cost_\N(f)/\cost_\A(f)$.

A {\em read-once (Boolean) formula} is a tree, each of whose internal nodes is labeled either $\vee$ or $\wedge$. The internal nodes  have 2 or more children. 
Each leaf is labeled with a Boolean variable $x_i \in \{x_1, \ldots, x_n\}$.  The formula computes a Boolean function in the usual way.\footnote{Some definitions of a read-once formula allow negations in the internal nodes of the formula.  By DeMorgan's laws, these negations can be ``pushed'' into the leaves of the formula,
resulting in a formula whose internal nodes are $\vee$ and $\wedge$, such that each variable $x_i$ appears in at most one leaf, possibly with negation.}

A {\em DNF formula} is a Boolean formula of the form $T_1 \vee T_2 \vee \ldots T_k$ for some $k \geq 1$, such that each $T_i$ is the conjunction ($\wedge$) of literals.  A literal is a variable $x_i$ or a negated variable $\neg x_i$.  The $T_i$ are called the {\em terms} of the DNF formula.   The DNF formula is read-once if distinct terms contain disjoint sets of variables, without negations.

A two-terminal series-parallel graph (TTSP) is a graph which includes two distinct, distinguished nodes $s$ and $t$ (called terminal nodes). It is defined recursively as follows. An edge is a TTSP, with endpoints $s$ and $t$.  A multi-graph $G$ with terminal nodes $s$ and $t$ is a TTSP if it is produced by combining two TTSPs, $G_1$ and $G_2$, either in series, or in parallel, as follows.  
Let $s_1$, $t_1$ and $s_2$, $t_2$, be the two terminal nodes of $G_1$ and $G_2$, respectively.
\begin{itemize}
    \item Parallel: $G$ is  produced by merging nodes $s_1$ and $s_2$ into the single node $s$, and  merging nodes $t_1$ and $t_2$ into the single node $t$.  (If this results in multiple copies of the same edge, all copies are preserved.)
    \item Series: $G$ is  produced by merging nodes $t_1$ and $s_1$ into a new single node, and by setting $s = s_1$ and $t=t_2$.
\end{itemize}
By ``merging nodes $v$ and $w$ into the single node $z$'' we mean that whenever $v$ or $w$ appears as an endpoint of an edge, it is replaced by $z$.  
If this results in the creation of identical edges, all copies are preserved, so that the total number of edges remains the same after the merge.  
Given a multi-graph $G=(V,E)$ with two distinct distinguished nodes $s$ and $t$, define the {\em $st$-connectivity function} $f:\{0,1\}^E \rightarrow \{0,1\}$ of the graph as follows.  Function $f$ is a Boolean function whose variables correspond to the edges of $G$. For any assignment $a \in \{0,1\}^E$, $f(a)=1$ if and only if there is an $s-t$ path in $G$ such that all edges in the path are set to 1 by $a$.  
A Boolean function $f$ is expressible by a read-once formula if and only if it is the $st$-connectivity function of a two-terminal series-parallel graph~\cite{RaghavanSchach90}.
\footnote{
Some authors use the term ``series-parallel'' more narrowly, to refer to a graph produced by combining parallel networks in series (see, e.g.,~\cite{kowshik2011information}).  The $st$-connectivity functions of these graphs correspond to read-once CNF formulas.} 

\subsection{Literature Review}

\href{https://people.cs.rutgers.edu/~sa1497/stuff/papers/stochastic_submodular-cover_2019.pdf}{Stochastic Submodular Cover with Limited Adaptivity}

\href{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8057094}{Complexity vs. Optimality: Unraveling
Source-Destination Connection in Uncertain Graphs}

\begin{itemize}
\item Read-Once DNF with Unit Costs and Uniform Probability:
$\Omega(\log n)$ lower bound and $O(\log n)$
\item Read-Once DNF with Unit Cost and Arbitrary Probability:
$\Omega(\sqrt{n})$ lower bound and $O(\sqrt{n})$
upper bound if constant length
\item Read-Once DNF with Arbitrary Cost and 
Uniform Probability: $\Omega(n^{1-\epsilon}/\log n)$
\item Read-Once Formula with Unit Cost and Constant Probability: $\Omega(\epsilon^3 n^{1-2\epsilon/\ln(2)})$ lower bound
\item DNF with Unit Costs and Uniform Probability:
$\Omega(n/\log n)$ lower bound
\end{itemize}


==> Adaptivity Gap/sections/results.tex <==
\section{Warm Up: Adaptivity Gaps for Read-Once DNFs}
\label{sec:read-once}

Let $f:\{0,1\}^n \rightarrow \{0,1\}$ be a read-once DNF formula.
Boros and \"{U}ny\"{u}lurt~\cite{BorosUnyulurt00} 
showed that the following approach gives an optimal adaptive
strategy for evaluating $f$
(this has been rediscovered in later papers~\cite{DBLP:journals/ai/GreinerHJM06,kowshik2011information,KaplanKM05}).
Let $f=T_1 \vee T_2 \ldots \vee T_k$ be a DNF formula with $k$ terms.  For each term $T_j$,
let $\ell(j)$ be the number of variables in term $T_j$.
Order the variables of $T_j$ as $x_{j_1}, x_{j_2}, \ldots x_{j_{\ell(j)}}$ in  non-decreasing order of the ratio $c_i /(1-p_i)$, i.e., so that 
$c_{j_1} /(1-p_{j_1}) \leq c_{j_2} /(1-p_{j_2}) \leq \ldots \leq c_{j_{\ell(j)}} /(1-p_{j_{\ell(j)}})$.
%We say $x_i \in T$ if variable $x_i$ is in term $T$. 
%Using this notation, let $P(T) = \prod_{x_i \in T} p_i$ and $C(T) = \sum_{x_i \in T} c_i$.
For evaluating the single term $T_j$, an optimal strategy
tests the variables in $T_j$ sequentially,
in the order $x_{j_1}, x_{j_2}, \ldots x_{j_{\ell(j)}}$, until a variable is found to be false, or until all variables are tested and found to be true.

Denote the probability of the term evaluating to true as $P(T_j) = \prod_{i=1}^{\ell(j)} p_{j_i}$ and the expected cost of this evaluation of the term
as $$C(T_j) = \sum_{i=1}^{\ell(j)} (\sum_{k=1}^i c_{j_k}\prod_{r=1}^{i-1} p_{j_r}).$$
%as $C(T_j) = c_j^1 + p_j^1 [c_j^2 + p_j^2 {\ldots}])$.
An optimal algorithm for evaluating $f$ applies the above strategy sequentially to the terms $T$ of $f$, in non-decreasing order of
the ratio $C(T)/P(T)$, until either some term is found to be satisfied by $x$,
so $f(x)=1$,
or all terms have been evaluated and found to be falsified by $x$,
so $f(x) =0$. 
%Consider $x_j$ for $j \in [|T_i|]$ which is the $j$th variable in $T_i$
%with associated probability of being true $p_j$ and cost of testing $c_j$.
%Once it tests within a term,
%the optimal adaptive strategy continues testing in non-decreasing order
%of $p_j/c_j$ until it finds a false variable or it certifies
%the term is true.
%Similarly,
%the optimal adaptive strategy tests terms in non-decreasing
%order of $P_i/C_i$ where $P_i = \prod_{j=1}^{|T_i|} p_j$
%and $C_i = \sum_{j = 1}^{|T_i|} c_j$.
%Since
%the optimal adaptive strategy may break ties arbitrarily,
%it follows there is always an optimal adaptive strategy which
%tests in a fixed order of terms and variables.
We will use this optimal adaptive strategy
in the remainder of the section.

In what follows, we will frequently describe non-adaptive strategies as performing the $n$ possible tests in a particular order.  We mean by this that the permutation representing the strategy lists the tests in this order.
The testing stops when the value of $f$ can be determined.
%\lisa{I wrote this, revising what was previously there, but don't think we need it}
%We will also use the associated non-adaptive strategy which 
%corresponds to the permutation produced by first
%listing the terms in non-decreasing order of $C(T)/P(T)$, and then
%replacing each term by listing the variables within it in non-decreasing order
%of $c_i/(1-p_i)$.  In terms of the tests performed, this strategy differs
%from the adaptive one in the following way: with the exception of the last term in the ordering,
%it will finish testing all variables within a term
%before moving on to the next term, rather than ``skipping'' the remaining variables in the term as soon as it finds an $x_i=0$.

%testing in the order of an optimal adaptive strategy
%without skipping the remaining variables in a term if a false variable is found.

\subsection{Unit Costs and the Uniform Distribution}

% \begin{lstlisting}[caption={Evaluating a read-once DNF where each variable has unit cost and uniform distribution.},label=alg:algorithm,captionpos=t,float,abovecaptionskip=-\medskipamount, mathescape=true,escapeinside={*}{*}]
%     Input: $n > 0$, read-once DNF $f:\{0,1\}^n \rightarrow \{0,1\}$ with $m$ terms
%     Output: $\pi$ # $O(\log n)$-approximate non-adaptive algorithm for $f$ 
%     $\pi \gets []$ # empty list
%     for $i$ in $[m]$ do
%         if $|T_i| \leq 2 \log n$ do # $T_i$ is $i$th shortest term in $f$
%             $\pi \gets \pi \text{ } + $ all variables in $T_i$
%         else do
%             $\pi \gets \pi \text{ } + $ first $2 \log n$ variables in $T_i$
%     $\pi \gets \pi \text{ } + $ remaining variables not in $\pi$
% \end{lstlisting}

\begin{algorithm}
    \DontPrintSemicolon
    \caption{Evaluating a read-once DNF where each variable has unit cost and uniform distribution.}\label{alg:algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}

    \Input{$n > 0$, read-once DNF $f:\{0,1\}^n \rightarrow \{0,1\}$ with $m$ terms}
    \Output{$\pi$ \tcp*{$O(\log n)$-approximation non-adaptive strategy for $f$}}
    $\pi \gets []$ \tcp*{empty list}
    \For{$i=1$ \KwTo $m$}{
        \eIf(\tcp*[f]{$T_i$ is $i$th shortest term in $f$}){$|T_i| \leq 2 \log n$}{$\pi \gets \pi \text{ } + $ all variables in $T_i$}{$\pi \gets \pi \text{ } + $ first $2 \log n$ variables in $T_i$}
    }
    $\pi \gets \pi \text{ } + $ remaining variables not in $\pi$
\end{algorithm}


We begin by showing that
the adaptivity gap for read-once DNFs, in the case of 
unit costs and the uniform distribution, 
is at most $O(\log n)$. 

\begin{theorem}\label{thm:rodnf-uu-upper}
Let 
$f:\{0,1\}^n \rightarrow \{0,1\}$ be a read-once DNF formula.
For unit costs and the uniform distribution,
there is a non-adaptive strategy $S$ such that 
$\cost(f,S) \leq O(\log n) \cdot \OPT_{\A}(f)$.
\end{theorem}

\begin{proof}[Proof Sketch]
Using the characterization of the optimal
adaptive strategy due to Boros and 
\"{U}ny\"{u}lurt~\cite{BorosUnyulurt00},
we show that Algorithm~\ref{alg:algorithm} gives
a non-adaptive strategy that has expected cost
at most $O(\log n)$ times
the optimal adaptive strategy.
The algorithm crucially relies on the observation
that the optimal adaptive algorithm tests 
terms in non-decreasing order of length for unit
costs and the uniform distribution.
To see this, observe $C(T)/P(T)$ is non-decreasing
when terms are ordered by length in this setting.
For terms with length at most $2 \log n$,
we can test every variable without paying more than
$O(\log n)$ times the optimal adaptive strategy.
For terms with length greater than $2 \log n$,
we can test $2 \log n$ variables and only need
to continue testing with probability $1/n^2$.
\end{proof}

We complement Theorem \ref{thm:rodnf-uu-upper}
with a matching lower bound.
We prove the theorem by exhibiting a read-once
DNF with $\sqrt{n}$ identical terms.
We upper bound the optimal adaptive strategy
and argue any non-adaptive strategy has to make
$\log n$ tests per term to verify $f(x)=0$ which
occurs with constant probability.

\begin{theorem}\label{thm:rodnf-uu-lower}
Let $f:\{0,1\}^n \rightarrow \{0,1\}$
be a read-once DNF formula.
For unit costs and the uniform distribution,
$\OPT_\N(f) \geq \Omega(\log n) \cdot \OPT_\A(f)$.
\end{theorem}

\subsection{Unit Costs and Arbitrary Probabilities}

We give an upper bound of the adaptivity gap for read-once DNF formulas
with unit costs and arbitrary probabilities 
in the special case where all terms
have the same number of variables.
This is known as a tribes formula \cite{ODonnellBook}.
Let the number of terms be $m$.
We now describe two non-adaptive strategies which yield
a $n/m$-approximation and a $m$-approximation, respectively.
Then, by choosing the non-adaptive strategy based on the
the number of terms $m$, we are
guaranteed a $\min \{n/m, m\} \leq O(\sqrt{n})$-approximation.

\begin{lemma}\label{lemma:n/m-approx}
    Consider a read-once DNF $f:\{0,1\}^n \rightarrow \{0,1\}$
    where each term has the same number of variables.
    For unit costs and arbitrary probabilities,
    there is a non-adaptive strategy $S \in \N$ such that $\cost(f,S) \leq n/m \cdot \OPT_\A(f)$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:n/m-approx}]
    Consider a random input $x$ and the optimal adaptive strategy described at the start of this section.
    If $f(x)=0$, the optimal adaptive strategy must
    certify that each term is 0 which requires at least
    $m$ tests.
    Since any non-adaptive strategy will make at most $n$
    tests, the ratio between the cost incurred on $x$ by a non-adaptive strategy, and by the optimal adaptive strategy, is at most $n/m$.
    Otherwise, if $f(x)=1$, the optimal adaptive strategy
    will certify that a term is true after testing some number
    of false terms. 
    Now consider the non-adaptive version of this optimal
    adaptive strategy which
    tests terms in the same fixed order but must test all variables in
    a term before proceeding to the next term.
    For each false term that the optimal adaptive strategy
    tests, the non-adaptive strategy will test every variable
    for a total of $n/m$ tests.
    Since the optimal adaptive strategy must make at least
    one test per false term,
    the ratio between the cost incurred on $x$ by the non-adaptive strategy, and the cost incurred by the optimal strategy, is at most $n/m$.  Since the ratio $n/m$ holds for all $x$, the lemma follows.
\end{proof}

\begin{lemma}\label{lemma:m-approx}
    Consider a read-once DNF $f:\{0,1\}^n \rightarrow \{0,1\}$
    where each term has the same number of variables.
    For unit costs and arbitrary probabilities,
    there is a non-adaptive strategy $S \in \N$ with
    expected cost $\cost(f,S) \leq m \cdot \OPT_\A(f)$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:m-approx}]
    Fix a random input $x$.
    If $f(x)=0$, the optimal adaptive strategy certifies
    that every term is false.
    Let $C_i$ be the number of tests it makes until
    finding a false variable on the $i$th term.
    Consider the non-adaptive ``round-robin''
    strategy which progresses in rounds,
    making one test in each term per round.
    Within a term, the non-adaptive strategy tests
    variables in the same fixed order as the optimal adaptive strategy.
    Then the cost of the non-adaptive strategy is
    $m \cdot \max_i C_i$ whereas the cost of the optimal adaptive
    strategy is $\sum_{i=1}^m C_i$.
    It follows that the adaptivity gap is at most $m$.
    Otherwise, if $f(x)=1$, the optimal adaptive strategy
    must certify that a term is true by making
    at least $n/m$ tests.
    Any non-adaptive strategy will make at most $n$ tests
    so the adaptivity gap is at most $m$.
\end{proof}

Together, the $O(n/m)$- and $O(m)$-approximations
imply the following result.

\begin{theorem}\label{thm:rodnf-ucap-upper}
    Let $f:\{0,1\}^n \rightarrow \{0,1\}$
    be a read-once DNF formula where each term has the same number of variables.
    For unit costs and arbitrary probabilities,
    there is a non-adaptive strategy $S \in \N$
    with $\cost(f,S) \leq O(\sqrt{n}) \cdot \OPT_\A(f)$.
\end{theorem}

We complement Theorem \ref{thm:rodnf-ucap-upper} with a matching lower bound.
We prove the theorem by exhibiting a read-once DNF
with $2\sqrt{n}$ identical terms.
By making one special variable in each term have a low
probability of being true and arguing it must always
be tested first, the non-adaptive strategy has to 
search at random for which special variable is true
when every other special variable is false which
happens with constant probability.

\begin{theorem}\label{thm:rodnf-ucap-lower}
Let $f:\{0,1\}^n \rightarrow \{0,1\}$
be a read-once DNF formula.
For unit costs and arbitrary probabilities,
$\OPT_\N(f) \geq \Omega(\sqrt{n}) \cdot \OPT_\A(f)$.
\end{theorem}

\subsection{Arbitrary Costs and the Uniform Distribution}

We prove Theorem \ref{thm:lambert} by exhibiting a
read-once DNF with $2^\ell$ terms each of length $\ell$.
Within each term, the cost of each variable increases
geometrically with a ratio of 2.
The challenge is choosing $\ell$ so that $2^\ell \ell = n$.
We accomplish this by using a modified Lambert W function 
\cite{bronstein2008algebraic}
which is how we calculate $n_\epsilon$.

\begin{theorem}\label{thm:lambert}
    For all $\epsilon > 0$, 
    there exists $n_{\epsilon} > 0$ such that the
    following holds for all read-once DNF formulas $f:\{0,1\}^n \rightarrow \{0,1\}$ where $n > n_{\epsilon}$: There exists a cost assignment such that for the uniform distribution,
    $\OPT_\N(f) \geq \Omega(n^{1-\epsilon}/\log n)
    \cdot \OPT_\A(f)$.
\end{theorem}

% We use the assumption in the theorem statement to show
% that $n$ must be greater than a modified 
% Lambert W function 
% for $n \ge n_\epsilon$.
% This will give the asymptotic behavior we claim.

\section{Main Result:
Read-Once Formulas}\label{sec:formula}

\begin{theorem}\label{thm:read-once-gap}
    Fix $\epsilon>0$.
    There is a read-once formula
    $f:\{0,1\}^n \rightarrow \{0,1\}$, such that
    for unit costs and $p_i=\frac{1+\epsilon}{2}$ for all $i \in [n]$,
    $\OPT_\N(f) \geq 
    \Omega\left(\epsilon^3 n^{1-2\epsilon/\log 2}\right)
    \cdot \OPT_\A(f)$.
\end{theorem}

Before we prove Theorem \ref{thm:read-once-gap},
we describe the read-once formula $f$ and
present the technical lemmas we use in the proof.
Without loss of generality, assume
$n=2 \cdot 2^d-2$ for some positive
integer $d$.
We define the function $f(x)$ on inputs $x\in \{0,1\}^n$
in terms of a binary tree with depth $d$. 
The edges of the tree are numbered $1$ through $n$,
and variable $x_i$  corresponds to edge $i$.
Each variable $x_i$ has a 
$\frac{1+\epsilon}{2}$ probability
of being true.
Say that a leaf of the tree is ``alive'' if
$x_i=1$ for all edges $i$ on the path from the root to the leaf.
We define $f(x)=1$ if and only if at 
least one leaf of the tree is alive.
A strategy for evaluating $f$ will continue testing until it can certify that there is at least one alive leaf, or that no alive leaf exists.
\begin{figure}[ht]
    \centering
    \includegraphics[scale=.16]{figures/branching_tree.pdf}
    \caption{The binary tree corresponding
    to the read-once formula we construct
    when $n=14$. In particular,
    $f(x)=(x_1\wedge((x_2\wedge(x_3\vee x_4))\vee(x_5\wedge(x_6\vee x_7))))\vee (x_8\wedge((x_9\wedge(x_{10}\vee x_{11}))\vee(x_{12}\wedge(x_{13}\vee x_{14}))))$.
    Notice that $f(x)=1$ for this $x$
    because the third leaf from the left is alive
    (all its ancestors are true).}
    \label{fig:branching_tree}
\end{figure}

Now consider the multi-graph that is produced from the tree
by merging all leaves into a single node.
The function $f$ is the $st$-connectivity function of this multi-graph.
It is easy to show, by induction on the depth of the tree, that the multi-graph is two-terminal series-parallel, with $s$ the root, and $t$ the node produced by merging the leaves of the tree.
Thus $f$ is computed by a read-once formula.  

We refer to the edges of the tree that join a leaf to its parent as leaf edges, and the other edges as internal edges.
 We say that a non-adaptive strategy $S$ is leaf-last if it first tests
all non-leaf edges of the tree, and then tests the leaf edges.  

In the proof of Theorem \ref{thm:read-once-gap},
we consider an alternative cost assignment where we pay unit costs for the tests on leaf edges, as usual, but tests on internal edges are free. 
%We use the term ``leaf-last'' to refer to the cost of a strategy under this cost assignment (it equals the number of leaf-edges tested).
The expected cost of a strategy under the usual unit cost assignment
is clearly lower bounded by its expected cost when internal edges are free.
Note that when internal edges are free,
there is no disadvantage in performing all the tests on internal edges first, so
there is an optimal non-adaptive strategy which is leaf-last
in the sense that all the leaf edges appear last.
Our first technical lemma describes a property of a leaf-last strategy.
We defer the proof of this lemma, and of the ones that follow, to the end of this section.
In all of the lemma statements, we assume $f$ is as just described, and expected costs are with respect to unit costs and test probabilities $p_i = \frac{1+\epsilon}{2}$.  We use $L$ to denote the number of leaves in the tree.

%Notice that the total number of tests can only be higher.
%Then, without loss of generality, the internal edges
%have already been tested for free
%and we want to lower bound the number
%of tests needed to evaluate the leaves.
%The next lemma describes a property of the optimal
%non-adaptive strategy that we will use to lower bound its cost.

\begin{lemma}\label{lemma:nonincreasingprob}
There exists a leaf-last non-adaptive strategy $S$ for evaluating $f$
which,
conditioned on the event that there is at least one alive leaf,
has minimum expected cost when internal edges are free relative to all non-adaptive strategies. Further, for any such $S$ and any $\ell \in [L-1]$, 
%$$\mbox{Pr(S first finds an alive leaf on the} \ell\mbox{th leaf test | there exists at least one live leaf} \geq 
%\mbox{Pr(S first finds an alive leaf on the} (\ell+1)\mbox{st leaf test | there exists at least one live leaf}$$ 
%Let $S$ be a non-adaptive strategy with minimum expected cost, relative 
 %that finds an alive leaf with the lowest
    %expected number of leaf tests conditioned
    %on the event that there is at least one alive leaf.
   % 
    conditioned on the existence of at least one alive leaf, the probability that $S$
    first finds an alive leaf on the $\ell$th leaf test
    is at least the probability $S$
    first finds an alive leaf on the
    $(\ell+1)$st leaf test. 
\end{lemma}

The next lemma gives us an
inequality that we will use to lower bound
the cost of the optimal non-adaptive strategy.

\begin{lemma}\label{lemma:earthmover}
    Let $L$ be a positive integer
    and $p_1 \geq p_2 \geq \ldots \geq p_L$
    be non-negative real numbers.
    %$p_\ell$ be a non-negative real number
    %for $\ell \in [L]$ such that 
    %$p_\ell \geq p_{\ell+1}$.
    Now let $p\geq p_1$ and define
    $L' = \lfloor \sum_{\ell=1}^L p_\ell/p \rfloor$.
    Then
    %\begin{align*}
    $
        \sum_{\ell=1}^L \ell p_\ell
        \geq \sum_{\ell=1}^{L'} \ell p.
    $
    %\end{align*}
\end{lemma}

Our analysis depends on there being at least constant probability that $f(x)=1$, or equivalently, that there is at least one alive leaf.
%
%The contribution to the expected
%cost of evaluating the leaves will only matter
%if there's a fixed probability that at least
%one alive leaf exists.
The next lemma assures us that this is indeed the case.  The proof of the lemma depends on our choice of having each $p_i$ be slightly larger than 1/2; it would not hold otherwise.  

\begin{lemma}\label{lemma:not2many}
% Consider a read-once formula 
% $f:\{0,1\}^n \rightarrow \{0,1\}$ and its
% binary tree representation.
With probability at least $\epsilon$,
there is at least one alive leaf in the binary tree representing $f$. 
\end{lemma}

With these key lemmas in hand, we prove
Theorem \ref{thm:read-once-gap}.

\begin{proof}[Proof of Theorem \ref{thm:read-once-gap}]
We will show that the adaptivity gap is large.
Intuitively, we rely on the fact that
if there is at least one alive leaf, 
then an adaptive strategy can find an alive leaf cheaply, 
by beginning at the root of the tree
and moving downward only along edges that are alive.
In contrast, a non-adaptive strategy cannot stop searching along
``dead'' branches.
However, it is not immediately clear that the cost of the
non-adaptive strategy is high because there are conditional
dependencies between the probabilities that two leaves with the same
ancestor(s) are alive.
To prove the desired result, we need to show that,
despite these dependencies, the optimal non-adaptive strategy
must have high expected cost.

We begin by showing that the expected cost
of any non-adaptive strategy is at least
$\frac{\epsilon^2}{16} n^{1-\frac{\epsilon}{\log 2}}$.
We want to lower bound the expected cost
of the optimal strategy $\OPT_\N(f)$:
\begin{align}\label{eq:dnf-leaf-cost}
    \min_{S \in \N} \E_{x}[\cost(f, x, S)]\geq
    \min_{S} \E[\cost^L(f, x, S)] =
    \min_{S'}
    \E[\cost^L(f, x, S')]
    %\E[\cost^L(S', x, S)]
\end{align}
where $\cost^L(f, x, S)$ is the number of
leaf tests $S$ makes on $x$ until
$f(x)$ is determined, and
$S'$ is a leaf-last strategy.
Then
\begin{align*}
    (\ref{eq:dnf-leaf-cost}) 
    &= \min_{S'} \left(
    \sum_{x:f(x)=1} \Pr(x) \cdot \cost^L(f, x, S')
    + \sum_{x:f(x)=0} \Pr(x) \cdot \cost^L(f, x, S')
    \right) \\
    &\geq \min_{S'}
    \sum_{x:f(x)=1} \Pr(x) \cdot \cost^L(f, x, S') \\
    &= \min_{S'}
    \sum_{\ell=1}^L \ell \Pr(\textrm{$S'$ first finds
    alive leaf on $\ell$th leaf test})
\end{align*}
where $L=2^d$ is the number of 
leaves in the binary tree.
Initially, all leaves have a $\left(\frac{1+\epsilon}{2}\right)^d$
probability of being alive
where $d = \log_2((n+2)/2)$.
By Lemma \ref{lemma:nonincreasingprob},
the probability that the next leaf is alive 
cannot increase as the optimal
non-adaptive strategy $S^*$ performs its test.
Set $$p=\left(\frac{1+\epsilon}{2}\right)^d$$ and 
$p_\ell = \Pr(\textrm{$S^*$ first finds
alive leaf on $\ell$th test})$.
Therefore, Lemma \ref{lemma:earthmover} with $p$ and $p_\ell$
tells us that 
\begin{align}\label{eq:binarynonlower}
    \sum_{\ell=1}^L \ell p_\ell
    \geq \sum_{\ell=1}^{L'} \ell 
    \left(\frac{1+\epsilon}{2}\right)^d
    \geq \left(\frac{1+\epsilon}{2}\right)^d
    \frac{\epsilon^2}
    {8\left(\frac{1+\epsilon}{2}\right)^{2d}}
    \geq \frac{\epsilon^2}
    {8 (\frac{n+2}{2})^{\log_2(\frac{1+\epsilon}{2})}}
    \geq \frac{\epsilon^2}{16} 
    n^{1-\frac{\epsilon}{\log 2}}
\end{align}
where we use the inequality that
$L' \geq \epsilon/(2\left(\frac{1+\epsilon}{2}\right)^d)$.
To see this,
recall that $\sum_{\ell=1}^L p_\ell/p \ge L'$
and, since the right-hand side is greater than 1,
$2L' \ge \sum_{\ell=1}^L p_\ell/p$.
By Lemma \ref{lemma:not2many},
$\sum_{\ell=1}^L p_\ell \ge \epsilon$ so
$L' \geq \epsilon/(2\left(\frac{1+\epsilon}{2}\right)^d)$.
The last inequality in Equation (\ref{eq:binarynonlower}) follows from
$\log_2(\frac{1+\epsilon}{2}) \leq \frac{\epsilon}{\log 2}-1$
which can be shown by comparing the $y$-intercepts
and derivatives for $\epsilon > 0$.

Next, we show that the expected cost
of the adaptive strategy is at most
$(n+1)^{\frac{\epsilon}{\log 2}}/\epsilon$.
Consider an adaptive strategy which starts by querying the
two edges of the root
and recurses as follows:
if an edge is alive it queries
its two child edges and otherwise stops.
Observe that this simple depth-first search
adaptive strategy will make at most two tests
for every alive edge in the binary tree.
Therefore the expected number of tests an adaptive
strategy must make is at most twice
the expected number of alive edges.
By the branching process analysis in the proof of Lemma
\ref{lemma:not2many},
twice the expected number of alive edges is
\begin{align}\label{eq:binaryadaptupper}
    2 \sum_{i=0}^d (1+\epsilon)^i
    \leq 2 \sum_{i=0}^{\log_2 n} (1+\epsilon)^i
    = 2 \frac{(1+\epsilon)^{\log_2 (n)+1}-1}
    {(1+\epsilon)-1}
    \leq 4 \frac{n^{\log_2(1+\epsilon)}}{\epsilon}
    \leq 4 \frac{n^{\frac{\epsilon}{\log 2}}}
    {\epsilon}
\end{align}
where the last inequality follows
from $\log_2(1+\epsilon) \leq \frac{\epsilon}{\log 2}$
which we can see by comparing the $y$-intercepts
and slopes for $\epsilon>0$.
Then Theorem \ref{thm:read-once-gap} follows
from Equations (\ref{eq:binarynonlower})
and (\ref{eq:binaryadaptupper}).
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:nonincreasingprob}]
    A leaf-last non-adaptive strategy $S$ satisfying the given conditional optimality property clearly exists, because any non-adaptive strategy can be made leaf-last by moving the leaf tests to the end without affecting its cost when internal edges are free.
    Define $p_\ell(S)$ as the probability that
    $S$ finds an alive leaf for the first
    time on leaf test $\ell$.
    We may write the expected number of
    leaf tests of $S$ as
    $\sum_{\ell=1}^L \ell p_\ell(S)$.
    
    Now suppose for contradiction that
    there is some $\ell'$ such that
    $p_{\ell'}(S) < p_{\ell'+1}(S)$.
    Let $S'$ be $S$
    but with the $\ell'$th and $(\ell'+1)$th
    tests swapped.
    We will show that the expected
    number of leaf tests made by $S'$
    is strictly lower than the expected
    number of leaf tests made by $S$.
    Observe that
    \begin{align*}
    \sum_{\ell=1}^L \ell p_\ell(S)
    - \sum_{\ell=1}^L \ell p_\ell(S')
    = \ell' (p_{\ell'}(S)-p_{\ell'}(S'))
    + (\ell'+1)(p_{\ell'+1}(S)-p_{\ell'+1}(S')).
    \end{align*}
    Notice that
    $p_{\ell'}(S) < p_{\ell'+1}(S) \leq p_{\ell'}(S')$
    where the first inequality
    follows by assumption
    and the second inequality follows
    because moving a test on a particular leaf edge to appear
    earlier in the permutation
    can only increase the probability
    that its leaf is the first alive leaf found.
    In addition, since
    the combined probability we first find an alive
    leaf in either the $\ell'$th or 
    $(\ell'+1$)th test is the same
    in either order of tests,
    $p_{\ell'}(S)+p_{\ell'+1}(S)
    = p_{\ell'}(S')+p_{\ell'+1}(S')$.
    Together,
    we have that
    $-(p_{\ell'}(S)-p_{\ell'}(S'))=
    p_{\ell'+1}(S)-p_{\ell'+1}(S')
    > 0$.
    Therefore
    $\sum_{\ell=1}^L \ell p_\ell(S)
    - \sum_{\ell=1}^L \ell p_\ell(S')=
    p_{\ell'+1}(S)-p_{\ell'+1}(S') > 0$
    and $S'$ makes fewer leaf tests
    in expectation even though $S$
    was optimal by assumption.
    A contradiction!
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:earthmover}]
Define $\delta_\ell = p - p_\ell \geq 0$
for $\ell \in [L']$.
Observe that $L' \leq L$ since
$p\geq p_\ell$ for all $\ell \in [L']$.
Then
\begin{align}\label{eq:delta_ell}
    \sum_{\ell=1}^L \ell p_\ell =
    \sum_{\ell=1}^{L'} \ell (p-\delta_\ell) +
    \sum_{\ell=L'+1}^L \ell p_\ell =
    \sum_{\ell=1}^{L'} \ell p
    - \sum_{\ell=1}^{L'} \ell \delta_\ell +
    \sum_{\ell=L'+1}^L \ell p_\ell.
\end{align}
Now all that remains to be shown is that
the sum of the last two terms in
Equation (\ref{eq:delta_ell}) is non-negative.
Notice that
\begin{align*}
    \sum_{\ell=1}^{L'} p_\ell
    + \sum_{\ell=L'+1}^{L} p_\ell \ge
    \sum_{\ell=1}^{L'} p
    \implies
    \sum_{\ell=L'+1}^L p_\ell \ge
    \sum_{\ell=1}^{L'} (p-p_\ell) =
    \sum_{\ell=1}^{L'} \delta_\ell.
\end{align*}
Then
\begin{align*}
    \sum_{\ell=1}^{L'} \ell \delta_\ell \leq
    L' \sum_{\ell=1}^{L'} \delta_\ell \leq
    L' \sum_{\ell=L'+1}^L p_\ell \leq
    \sum_{\ell=L'+1}^L \ell p_\ell.
\end{align*}
\end{proof}

\begin{proof}[Proof of Lemma \ref{lemma:not2many}]
Let $Z_i$ denote the number of alive
edges at level $i$.
Then the statement of Lemma \ref{lemma:not2many} becomes 
$\Pr(0< Z_d) \geq \epsilon$.
Using standard results from the study of branching
processes, we know that
\begin{align*}
  \E[Z_d] = \mu^d
  \hspace{1em} \textnormal{ and } \hspace{1em}
  \Var{Z_d} = \left(\mu^{2d} - \mu^{d} \right)
  \frac{\sigma^2}{\mu (\mu-1)}
\end{align*}
where
$\mu$ is the expectation
and $\sigma$ is the variance
of the number of alive ``children'' from a single alive edge
(see e.g., p. 6 in Harris \cite{harris1963theory}).
In our construction,
\begin{align*}
   \mu = 2\left(\frac{1+\epsilon}{2}\right)
    = (1+\epsilon)
   \hspace{1em} \textnormal{ and } \hspace{1em}
   \sigma^2 
   = 2\left(\frac{1+\epsilon}{2}\right)
   \left(1-\frac{1+\epsilon}{2}\right)
   =\frac{1-\epsilon^2}{2}
\end{align*}
since the children of one edge follow the binomial
distribution.
Then $\E[Z_d] = (1+\epsilon)^d$
and
\begin{align*}
    \Var{Z_d} = \left( (1+\epsilon)^{2d}
    - (1+\epsilon)^d \right)
    \frac{1-\epsilon^2}{2(1+\epsilon)\epsilon}
    \leq \frac{1}{2\epsilon}
    \left((1+\epsilon)^{d}\right)^2
    = \frac{1}{2\epsilon} \E[Z_d]^2.
\end{align*}

We will now use Cantelli's inequality
(see page 46 in Boucheron et al. \cite{boucheron2013concentration})
to show that $\Pr(Z_d > 0) \geq \epsilon$.
Cantelli's tells us that 
$\Pr(X - \E[X] \geq \lambda) 
\leq \frac{\Var{X}}{\Var{X}+\lambda^2}$
for any real-valued random variable $X$ and 
$\lambda > 0$.
Choose $X= -Z_d$ and $\lambda = \E[Z_d]$.
Then
\begin{align*}
    \Pr(Z_d \leq \E[Z_d] - \E[Z_d])
    \leq \frac{\Var{Z_d}}{\Var{Z_d}+\E[Z_d]^2}
\end{align*}
and, by taking the complement,
\begin{align}\label{eq:applied-cantelli}
    \Pr(Z_d > 0) \geq 
    \frac{\E[Z_d]^2}{\Var{Z_d}+\E[Z_d]^2}
    \geq \frac{\E[Z_d]^2}
    {\frac{1}{2\epsilon}\E[Z_d]^2
    +\E[Z_d]^2} = \frac{2\epsilon}{1+2\epsilon}
    \geq \epsilon
\end{align}
for $0 < \epsilon \leq 1/2$.
%Next, using Chebyshev's inequality,
%we will show that 
%$\Pr\left(Z_d \geq
%(1+\frac{1}{\epsilon})\E{Z_d}\right)
%\leq \frac{\epsilon}{2}$.
%Chebyshev's tells us that
%$\Pr(|Z_d - \E{Z_d}| \geq \lambda)
%\leq \Var{Z_d}/\lambda^2$.
%Then,
%taking only the positive part
%of the absolute value
%with $\lambda=\E{Z_d}/\epsilon$,
%we have that
%\begin{align}\label{eq:applied-chebyshev}
%    \Pr \left(Z_d \geq 
%    \left(1+\frac{1}{\epsilon}\right)
%    \E{Z_d}\right)
%    \leq \frac{\frac{1}{2\epsilon}\E{Z_d}^2}
%    {\frac{1}{\epsilon^2}\E{Z_d}^2} =
%    \frac{\epsilon}{2}.
%\end{align}
Then Lemma \ref{lemma:not2many}
follows from Equation (\ref{eq:applied-cantelli}).
\end{proof}


\section{DNF Formulas}
\label{sec:dnf}

We will show near-linear and linear in $n$ lower 
bounds for DNF formulas under the uniform distribution with
unit and arbitrary costs, respectively.
Since the function we exhibit has linear terms,
the lower bounds also apply to the class of linear-size DNF formulas.

\begin{theorem}\label{thm:nlognlower}
Let $f:\{0,1\}^n \rightarrow \{0,1\}$
be a DNF formula.
For unit costs and the uniform distribution,
$\OPT_\N(f) \geq \Omega(n/\log n) \cdot \OPT_\A(f)$.
\end{theorem}

\begin{proof}
Without loss of generality,
assume $n=2^d + d$ for some positive integer $d$.
Consider the address function $f$ with
$2^d$ terms which each consist of
$d$ shared variables appearing in all terms, and a
single dedicated variable appearing only in that term.
%For shorthand, let $\overline{x}_i=1-x_i$.
We may write $f = T_0\vee T_1\vee\cdots\vee T_{2^d-1}$
where $T_i$ consists of the shared variables
negated according to the binary representation of $i$
and the single dedicated variable.
%\begin{align*}
%    T_1 &= (\overline{x}_d\wedge \overline{x}_{d-1}\wedge 
%    \dots \wedge \overline{x}_2 \wedge \overline{x}_1 \wedge x_{d+1})\\
%    T_2 &= (\overline{x}_d\wedge \overline{x}_{d-1}\wedge 
%    \dots \wedge \overline{x}_2 \wedge x_1 \wedge x_{d+2})\\
%    T_3 &= (\overline{x}_d\wedge \overline{x}_{d-1}\wedge 
%    \dots \wedge x_2 \wedge \overline{x}_1 \wedge x_{d+3})\\
%    & \vdots \\
%    T_{2^d} &= (x_d\wedge x_{d-1}\wedge
%    \dots \wedge x_2 \wedge x_1\wedge x_{d+2^d})
%\end{align*}

By testing the $d$ shared variables, the optimal
adaptive strategy can learn which single term
is unresolved and test the corresponding dedicated
variable in a total of $d+1$ tests.
In contrast, any non-adaptive strategy has to search
for the unresolved dedicated test at random which
gives expected $2^d/2$ cost.
(We can ensure the non-adaptive strategy tests
the shared variables first by making them free which can
only decrease the expected cost.)
It follows that the adaptivity gap
is $\Omega(2^d/d) = \Omega(n/\log n)$.
\end{proof}

%\begin{theorem}\label{thm:nlognupper}
%Let $f:\{0,1\}^n \rightarrow \{0,1\}$
%be a Boolean formula.
%For unit costs,
%there is a non-adaptive strategy
%$S \in \N$ with cost
%$\cost(f,S) \leq O(n/\log n) \cdot \OPT_\A(f)$.
%\end{theorem}
%
%As mentioned in the acknowledgements,
%we would like to thank an anonymous reviewer
%for the following proof of Theorem
%\ref{thm:nlognupper}.
%
%\begin{proof}
%If the expected cost of the optimal adaptive strategy
%is at least $\log n/2$, then the non-adaptive
%strategy pays at most $n$ since each test is unit cost
%and the adaptivity gap is at most $O(n /\log n)$.
%Otherwise, the expected cost of the
%optimal non-adaptive strategy is
%$c \log n /2$ for some $c < 1.$
%By Markov's inequality, we know the probability
%the adaptive strategy pays more than $\log n/2$ is $c$.
%In $\log n/2$ tests, the adaptive strategy
%can test at most $\sqrt{n}$ different variables.
%Consider the non-adaptive strategy that 
%tests those $\sqrt{n}$ variables then
%randomly tests the remaining variables.
%The expected cost of this strategy is $\sqrt{n} + cn$
%so the adaptivity gap is $O(n /\log n)$.
%\end{proof}

We can easily modify the address function
in the proof of Theorem \ref{thm:nlognlower}
to prove an $\Omega(n)$ lower bound
for DNF formulas under the uniform
distribution and arbitrary costs.
In particular, make the cost of each shared variable $1/d$.
Then the adaptive strategy
pays $d\cdot(1/d) + 1=2$
while the non-adaptive strategy still
pays $\Omega(n)$.
The $O(n)$ upper bound comes from the
increasing cost strategy and analysis in
\cite{DBLP:conf/stoc/KaplanKM05}.

\begin{theorem}\label{thm:nlower}
Let $f:\{0,1\}^n \rightarrow \{0,1\}$
be a DNF formula.
For the uniform distribution,
$\OPT_\N(f) \geq \Theta(n) \cdot \OPT_{\A}(f)$.
\end{theorem}



\section{Conclusion and Open Problems}

We have shown bounds on the adaptivity gaps 
for the SBFE problem for well-studied classes of Boolean formulas.
Our proof of the lower bound for read-once formulas depended on having $p_i$'s that are slightly larger than 1/2 but we conjecture that a similar or better lower bound holds for the uniform distribution.  
We note that our lower bound for read-once formulas also applies to (linear-size) monotone DNF formulas, since the given read-once formula based on the binary tree has a DNF formula with one term per leaf.  Another open question is to prove a lower bound for monotone DNF formulas that matches our lower bound for general DNF formulas.  

A long-standing open problem is whether the SBFE problem for read-once formulas has a polynomial-time algorithm (cf.~\cite{DBLP:journals/ai/GreinerHJM06,Unluyurt04}).
The original problem only considered adaptive strategies, and it is also open whether there is a
polynomial-time (or pseudo polynomial-time) constant or $\log n$ approximation algorithm for such strategies.
Happach et al.~\cite{happach2021general} gave a pseudo polynomial-time approximation algorithm 
for the non-adaptive version of the problem, which outputs a non-adaptive strategy with expected cost within a constant factor of the optimal non-adaptive strategy.
Because of the large adaptivity gap for read-once formulas,
as shown in this paper, the result of Happach et al.
does not have any implications for the open question
of approximating the adaptive version of the SBFE
problem for read-once formulas.
%If the adaptivity gap for read-once formulas were e.g., logarithmic, then this would have implied a log-factor pseudo polynomial-time approximation algorithm for the adaptive version of the problem.
%The large adaptivity gap shown in this paper tells us that no such implication holds, and the question of approximating the original adaptive version of the SBFE problem for read-once formulas remains open.

%Open problems:
%\begin{itemize}
  %  \item Upper bound for read-once DNF
  %  with unit cost arbitrary probability
  %  when number of variables in each term is not
  %  cosntant
  %  \item Adaptivity gaps for other classes
  %  of functions?
    % \item For the functions which we are not able to prove an $\Omega(n)$ adaptivity gap, can we find a matching upper bound or can we improve our lower bound?
    % \item Can we find a PTAS for the SBFE problem?
%\end{itemize}


==> sections/draft.tex <==
\paragraph{Papers with adaptivity gap techniques:}
\begin{itemize}
    \item \href{https://link.springer.com/article/10.1007/s10107-015-0927-9}
    {On the Adaptivity Gap of Stochastic Orienteering (Bansal, Nagarjan)}:
    Uses binary tree construction to get lower bound.
    \item
    \href{https://arxiv.org/pdf/1608.00673.pdf}
    {Adaptivity Gaps for Stochastic Probing:Submodular and XOS Functions (Gupta, Nagarajan, Singla)}:Improves on results of Asadpour et al. and others.  Gives constant-factor adaptivity gap for maximizing monotone submodular fn subject to a very general class of constraints, called prefix-closed constraints (including matroid constraints, knapsack constraints, cardinality constraints). 
    They survey previous techniques including e.g.: use LP relaxations to lower bound optimal cost of adaptive strategy, use multilinear extension of submodular fns -- and then try to find a non-adaptive strategy that is close to this lower bound.  Instead, they take an adaptive strategy and show that you can get a non-adaptive strategy from it with low expected cost (not much more than the adaptive strategy) by randomly choosing a root-leaf path as your non-adaptive strategy.  And this shows that a non-adaptive strategy with low expected cost exists. 
    \item \href{https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.142.9979&rep=rep1&type=pdf}{Stochastic Submodular Maximization. (Asadpour, Nazerzadeh)}: using Poisson clock
    \item \href{https://theory.stanford.edu/~jvondrak/data/knapsack_focs.pdf}{Approximating the Stochastic Knapsack Problem: The Benefit of Adaptivity (Dean, Goemans, Vondrak)}
    \item \href{https://researcher.watson.ibm.com/researcher/files/us-jvondrak/stoch_cover.pdf}{Stochastic covering and adaptivity. (Goemans, Vondrak)}
    \item \href{https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.481.772&rep=rep1&type=pdf}{Adaptivity and Approximation for Stochastic Packing Problems (Dean, Goemans, Vondrak)}:
    Uses construction to get lower bound.
    \item
    \href{https://arxiv.org/abs/1504.02146}{Discrete Stochastic Submodular Maximization: Adaptive vs. Non-adaptive vs. Offline (Hellerstein, Kletenik, Lin)}: Starts with an adaptive tree and proves that you can collapse it into a single path (non-adaptive strategy) in such a way that the resulting expected cost isn't too much bigger than the expected cost of the original tree.  The bound obtained depends on the $p_i$'s.  
\end{itemize}

\teal{Upper bound of adaptivity gap is number of variables
from increasing greedy cost non-adaptive strategy.}

\teal{Say unit cost}

\teal{Add what we know about symmetric functions.}

\teal{$O(k)$ upper bound on adaptivity gap where $k$
is number of terms in a read once DNF.
Adaptive strategy can either keep querying the same term
or move to another.
We know what term it will query in each term
(highest probability of resolving / cost), so if 
we round robin between terms then we get $O(k)$
times adaptive.}

\lnf{
The adaptivity gap was first introduced in the study of stochastic knapsack problem by Dean et al.~\cite{DBLP:conf/focs/DeanGV04}, and in that particular problem they showed the adaptivity gap is 8, and later Bhalgat~\cite{bhalgat2+} improved it to $2+\varepsilon$. Dean et al.~\cite{DBLP:conf/soda/DeanGV05} generalized it to the stochastic packing problem, in which they allow the knapsack constraints to be multidimensional. Gupta et al.~\cite{DBLP:conf/soda/GuptaNS16} study the stochastic probing problem and gave a $O(\log n)$ adaptivity gap. Later Gupta et al.~\cite{DBLP:conf/soda/GuptaNS17} improved it to 3 and Bradac et al.~\cite{DBLP:conf/approx/Bradac0Z19} improved it to 2, which is close to the lower bound $\frac{e}{e-1}$ given by Asadpour et al.~\cite{DBLP:conf/wine/AsadpourNS08}. Fu et al.~\cite{DBLP:conf/icalp/FuLX18} gave a PTAS for a class of stochastic dynamic programs, which include the probing problem and variants of the stochastic knapsack problem. Although the adaptivity gaps for stochastic maximization problems are well studied, there has been little progress on stochastic minimization problems. Goemans et al.~\cite{DBLP:conf/latin/GoemansV06} study the stochastic covering problem, and they showed if the items can be used repeatedly, the adaptivity gap is $\Theta(\log d)$ where d is the size of target set to be covered. They also pointed out the adaptivity gap can be arbitrarily large if the items can be used only once. Recently Ghuge et al.~\cite{Ghuge21} showed constant the adaptivity gap for the stochastic score classification problem, which was previously introduced by Gkenosis et al.~\cite{gkenosisetal18}. All those results make us wondering what is the adaptivity gap for the SBFE problem.
}


%\section{Monotone DNF}
%
%\begin{theorem}
%There is a monotone DNF
%with $N$ terms and $N + 2\log_2 N$ variables
%where the optimal non-adaptive
%strategy has expected cost $\Omega(N^{.32})$
%times the optimal adaptive strategy.
%\end{theorem}
%
%\begin{proof}
%
%\item \paragraph{Construction}
%
%The monotone DNF construction is equivalent to the DNF
%construction except that we replace $\overline{x}_i$ with
%a new independent variable $x_i'$.
%Additionally, each $x$-variable is still 1 with probability 1/2
%but each $y$-variable is 1 with probability 1.
%\teal{We'll eventually talk about extending to the
%uniform setting so our lower bound result is stronger.}\lnf{I agree, and I'll work on this tonight.}
%
%\item \paragraph{Adaptive Expected Cost}
%
%We argue that the optimal adaptive strategy tests the $x$
%variables before testing any of the $y$-variables since each
%$x$-variable gives information about strictly more
%terms than any $y$-variable.
%Without loss of generality, we test in order of increasing index.
%If $x_i=1$, we continue to $x_{i+1}$.
%If $x_i=0$, we test $x_i'$ since there's a $(1-p)^2$ probability
%we will immediately find a 0-certificate.
%
%If we test all of the $x$-variables without finding a 0-certificate,
%then we know exactly which terms have only 1's and with a single
%additional test we will have a 1-certificate.
%
%Using this optimal strategy, 
%we can generate the following decision tree:
%Let $c(n)$ denote the expected cost of the optimal decision tree with $n$ of $x_i$ (also $n$ of $x_i'$ and $2^n$ of $y_i$),
%we can write the following:
%\begin{align*}
%    c(n) = p\cdot c(n-1) + (1-p)\cdot (p\cdot c(n-1)+1) + 1
%\end{align*}
%
%Since $p=0.5$, we have
%\begin{align*}
%    c(n) &= 0.5\cdot c(n-1) + 0.5\cdot (0.5\cdot c(n-1)+1) + 1\\
%    &=0.75\cdot c(n-1)+1.5\\
%    c(n)-6 &= 0.75\cdot (c(n-1) -6)
%\end{align*}
%
%Hence, $c(n)$ converges to 6 when $n\rightarrow \infty$
%and the expected cost of the optimal adaptive strategy
%is constant.
%
%\item \paragraph{Non-Adaptive Expected Cost}
%
%We do not know what the optimal non-adaptive strategy
%is but we argue that it tests all the $x$-variables
%before any of the $y$-variables for the same reason
%as the optimal adaptive strategy.
%If there is a 0-certificate then the non-adaptive strategy
%also has constant expectation.
%If there is a 1-certificate then the non-adaptive strategy
%will test all of the $x$-variables and then
%need to find a $y$-variable in a term with only 1's.
%The high-level idea is that finding such a $y$-variable
%is difficult for the non-adaptive strategy.
%
%Formally,
%we argue that the expected cost of finding a 1-certificate
%is very high.
%In order to lower bound this expectation, we partition
%assignments with 1-certificates based on the number of
%pairs $t$ where $x_i=x_i'=1$ for $i \in [n]$.
%The probability that there are $t$ pairs is
%$\binom{n}{t} (1/4)^t (1/2)^{n-t}$ since there's a $1/4$ probability
%pair $i$ has $x_i=x_i'=1$, a $1/2$ probability either
%$x_i=1$ or $x_i'=1$, and $\binom{n}{t}$ ways to choose
%these pairs.
%
%The expected cost of a non-adaptive strategy finding a
%term with a 1-certificate is
%$(2^n+n)/2^{t+1} \geq 2^{n-t-1}$ by the following argument.
%
%Say that an assignment to the $x_i, x_i'$ pairs is a `t-assignment' if
%\begin{enumerate}
%    \item for $t$ of the $x_i,x_i'$ pairs, $x_i=x_i'=1$, and
%    \item for the other $n-t$ pairs, exactly one 
%    of $x_i$ and $x_i'$ is equal to 1.
%\end{enumerate}
%
%Consider any non-adaptive ordering of the $y$-variables.
%Without loss of generality, we relabel the variables so
%the non-adaptive ordering is
%$y_1,y_2,...,y_{N}$ with corresponding terms
%$t_1,\ldots,t_{N}$.
%
%Let $A$ be a random $t$-assignment, chosen uniformly
%from all $t$-assignments.
%%(as before, we assume
%%that all $y$-variables are set to 1 in this assignment).
%Let $c(A)$ denote the number of tests on $y$-variables
%that are performed on $A$ according to a non-adaptive strategy.
%We want to show a lower bound on the expected value of $c(A)$.
%
%The value of $c(A)$
%is the unique index $i$ such that $A$ 
%does not satisfy the terms associated 
%with $y_1,..,y_{i-1}$,
%but $A$ does satisfy the term associated with $y_i$.
%
%Let $Z = \binom{n}{t}$. There are $Z*2^{n-t}$ total $t$-assignments.
%For any particular $i$, term $t_i$ is satisfied by
%exactly $Z$ many of these $t$-assignments.
%Thus the probability that $A$ satisfies a particular term $t_i$
%is $Z / (Z*2^{n-t})$ = $1 / (2^{n-t})$.
%It follows from a Union Bound that for any particular $i$,
%the probability that $A$ satisfies $t_1$ or $t_2$ or ... or $t_i$
%is less than $i / 2^{n-t}$.
%
%Therefore,
%\begin{align*}
%    \Pr(c(A) > i ) \geq 1 - \frac{i}{2^{n-t}}.
%\end{align*}
%
%Now consider a random variable $X$ that takes values
%in $[2^{n-t}]$ with uniform probability. 
%For each $i$ in the support of $X$,
%$\Pr(X > i) = 1 - i / 2^{n-t}$.
%Since $X$ is equally likely to take any value between 1 and
%$2^{n-t}$, its expected value is $2^{n-t}/2$.
%Observe that
%$\Pr(c(A) > i) \geq \Pr(X > i)$
%for all $i \in [n]$.
%Therefore the expected value of $c(A)$ is
%lower bounded by the expected value of $X$ which is $2^{n-t}/2$.
%
%Then the expected cost of any non-adaptive strategy
%finding a 1-certificate is at least
%\begin{align*}
%    \frac{1}{2} \sum_{t=0}^n 
%    \binom{n}{t} (1/4)^t (1/2)^{n-t} (2^{n-1})
%    = \frac{1}{2} \sum_{t=0}^n 
%    \binom{n}{t} (1/4)^t = (1+1/4)^n
%\end{align*}
%where the last equality follows from the observation that
%the sum is an ordinary generating function of the binomial
%sequence.
%Using $n = \log_2 N$,
%we get that the expected cost is
%$N^{\log_2 5/4} \approx N^{.32}$.
%
%\end{proof}

%Although we don't know what's exactly the optimal non-adaptive strategy, 
%we can lower-bound it. 
%We use conditional expectation here. 
%Let $\E{\OPT}$ denote the optimal non-adaptive strategy, then we let $\E{\OPT\mid g=i}$ to denote the expected cost to evaluate the function when there are $i$ terms being 1 and $p_i$ to be the probability that there are $i$ terms being 1.
%Hence, we have the following
%\begin{align}
%    \E{\OPT} = \sum_{i=0}^{2^n}\E{\OPT\mid g=i}\cdot p_i \label{eq:1}
%\end{align}
%
%We first take a look at $p_i$. Notice that
%\begin{itemize}
%    \item When $i=1$, it means \textit{only one of each $\{x_i, x_i'\}$ is 1}. Hence, $p_1=\frac{1}{2}^n$.
%    \item When $i=2$, it means \textit{only one of each $\{x_i, x_i'\}$ is 1, except there exist one pair that both of $\{x_i, x_i'\}$ are 1}. Hence, $p_2=(\frac{1}{2})^{n-1}\cdot\frac{1}{4}\cdot {n\choose 1}$.
%    \item When $i=3$, $p_3=0$ since it's only possible to have $2^{k}$ terms to be one, where $k\in\{0,1,\dots,n\}$.
%\end{itemize}
%
%Hence we can rewrite part of (\ref{eq:1}) to the following:
%\begin{align}
%    \E{\OPT \mid g\geq 2}\cdot p_{g\geq 2} &= \sum_{i=1}^{t}\E{\OPT\mid g=2^t}\cdot p_{2^t}\notag\\
%    &=\sum_{t=1}^{n}\E{\OPT\mid g=2^t}\cdot (\frac{1}{2})^{n-t}\cdot\frac{1}{2}^{2t}\cdot {n \choose t}\label{eq:2}
%\end{align}
%
%Next we deal with $\E{\OPT\mid g=i}$.
%\begin{itemize}
%    \item When $i=1$, $\E{\OPT\mid g=i}=\frac{1}{2}\cdot 2^n$
%    \item When $i=2$, $\E{\OPT\mid g=i}=\frac{1}{2}\cdot 2^{n-1}$
%    \item When $i=4$, $\E{\OPT\mid g=i}=\frac{1}{2}\cdot 2^{n-2}$
%\end{itemize}
%
%Hence, $\E{\OPT\mid g=i}=2^{n-i-1}$. Apply this to (\ref{eq:2}) we have the following:
%\begin{align}
%    (\ref{eq:2})=\sum_{t=1}^n 2^{n-t-1}\cdot (\frac{1}{2})^{n-t}\cdot\frac{1}{2}^{2t}\cdot {n \choose t} := \sum_{t=1}^n h(t)\label{eq:3}
%\end{align}
%
%When $t=1$,
%\begin{align*}
%    h(1)=2^{n-2-n+1-2}\cdot n = (\frac{1}{2})^3\cdot n
%\end{align*}
%
%Hence, $\E{\OPT} = \Omega(n)=\Omega(\log N)$.
%

\section{Notes for 7/14}
\begin{itemize}
    \item The non-monotone DNF also works for polynomial-size decision tree.
    \item open problems
    \begin{itemize}
        \item is the adaptivity gap for arbitrary Boolean function $\Omega(n)$?\\
        \lnf{for arbitrary cost, I think yes. By replacing the unit-cost of $y_i$ with a large cost will yields adaptivity gap of $\Omega(n)$}
        \item Is the adaptivity gap for arbitrary monotone functions
less than it is for arbitrary non-monotone Boolean functions?
Can you show e.g. that the gap is no more than O(sqrt(N))
for the uniform distribution and unit costs?
    \end{itemize}
\end{itemize}

\section{Symmetric functions}
\begin{itemize}
    \item Upper bound of symmetric function with unit cost is 2. \lnf{actually 4, according to the previous error}
    \item Upper bound of symmetric function with arbitrary cost is something close to 8 (CHECK THIS). 
\end{itemize}

==> sections/intro_old.tex <==
\section{Introduction}

We consider the question of determining adaptivity gaps for Stochastic Boolean Function Evaluation (SBFE) problems. Fix a positive integer $n$. In the SBFE problem for a Boolean function $f:\{0,1\}^n \rightarrow \R $, we are given a (representation of) a Boolean function $f(x_1, \ldots, x_n)$ and asked to determine the value of the function on an initially unknown random input $x=(x_1,\ldots, x_n)$.  The values of the individual variables $x_i$ are independent, and for each $x_i$, we are given $p_i=P[x_i=1]$.
The value of an $x_i$ in $x$ can only be determined by performing a ``test''. Testing $x_i$ incurs a given cost $c_i$, and tests must be performed sequentially.  Testing continues until the value of $f(x)$ can be determined.  The problem is to determine the order in which to perform the tests, so as to minimize the total expected cost of the tests.  The testing order can be adaptive, meaning that the choice of the next test $x_i$ can depend on the outcome of previous tests. An adaptive test ordering, often called a ``strategy,'' corresponds to a decision tree.

An interesting example of an SBFE problem is 
determining $st$-connectivity in uncertain networks, a problem defined by Fu et al.\cite{DBLP:journals/ton/FuFXPWL17} \lisa{check reference}.  The input to the problem is a graph $G$ with source node $s$ and destination node $t$, and for each edge, a cost $c_e$ and a probability $p_e$. 
Each edge $e$ in the graph is either ``usable'' or ``unusable''.
Edge $e$ is usable with independent probability $p_e$.
The only way to determine whether edge $e$ is usable is to perform a test with cost $c_e$.
The problem is to determine the order in which to perform tests 
so as to minimize the expected cost of determining whether 
there is a path of usable edges from $s$ to $t$.
This is an SBFE problem for a Boolean function $f$, defined by $G$, $s$, and $t$, whose input variables correspond to the edges in $G$,
and whose output is positive if and only if there is a path from $s$ to $t$
whose associated edge variables are all positive.
We call such a function $f$ an $st$-connectivity function.
Thus the problem of determining $st$-connectivity in an uncertain network is equivalent to the SBFE problem for $s$-$t$ connectivity functions $f$.
%such that the value of $f$ on an input assignment is 1 if and only if there is an $s$-$t$
%path in $G$ whose corresponding edge variables are all set to 1.

In some practical settings, it is desirable to consider only ``non-adaptive'' testing strategies.  A non-adaptive testing strategy is a permutation of the tests; testing continues in the order specified by the permutation until no more testing is needed (here, until the value of $f(x)$ can be determined).
A non-adaptive strategy corresponds to an adaptive strategy whose decision tree representation has the property that all non-leaf nodes on the same level contain the same test $x_i$.

The ``adaptivity gap'' is a measure of how much benefit can be obtained from adaptivity.
Let $\cost_\N(f)$ be the minimum expected cost
of evaluating $f$ over non-adaptive strategies
and $\cost_\A(f)$ be the minimum expected cost
of evaluating $f$ over adaptive strategies.
% The adaptivity gap of the SBFE problem for $f$ is
% $\cost_\N(f)/\cost_\A(f)$.
Let $F$ be a class of Boolean functions, and let $F_n$
denote the functions in $F$ with $n$ input variables.
The adaptivity gap of the SBFE problem for the class $F$ 
is the function $g:\mathcal{N} \rightarrow \mathcal{R}$
such that for all $n \in \mathcal{N}$, 
$g(n) = \max_{f \in F} \cost_\N(f)/\cost_\A(f)$.

It is well-known that the SBFE problem for the Boolean OR function given by $f(x_1, \ldots, x_n) = x_1 \vee \ldots \vee x_n$ has a simple solution:  
test the variables $x_i$ in increasing order of the ratio $c_i/p_i$ until finding some variable is positive, or all variables are found to be negative. This strategy is non-adaptive, meaning that the SBFE problem for the Boolean OR function has an adaptivity gap of 1.  That is, there is no benefit to adaptivity.  

It is also known that, for arbitrary Boolean functions, the non-adaptive strategy of testing the $x_i$ in increasing order of $c_i$ has an expected cost that is within a factor of $n$ of the optimal adaptive strategy~\cite{DBLP:conf/stoc/KaplanKM05}\lisa{add cite}. Thus the adaptivity gap for the SBFE problem on any class of Boolean functions is somewhere between 1 and $n$.  

In this paper we prove adaptivity gaps for the SBFE problem on (the class of functions) associated with three well-studied classes of Boolean formulas:

\begin{table}[]
\centering
\caption{A summary of our results.
*Indicates the upper bound only applies for
read-once DNFs where every term has the same
number of variables.}
{\renewcommand{\arraystretch}{1.2}
\begin{tabular}{|l|l|l|l|}
 \hline
 \textbf{Formula Class} & \textbf{Costs} 
 & \textbf{Probabilities} & \textbf{Adaptivity Gap} \\
\hline
Read-once DNF & Unit & Uniform & $O(\log n)$ and $\Omega(\log n)$ \\
\hline 
Read-once DNF & Unit & Arbitrary & $O(\sqrt{n})$* and $\Omega(\sqrt{n})$ \\
\hline
Read-once DNF & Arbitrary & Uniform & $\Omega(n/\log n)$ \\
\hline
Read-once Formula & Unit & Constant & $\Omega(\epsilon^3 n^{1-2\epsilon/\ln(2)})$ \\
\hline
Non-Monotone DNF & Unit & Uniform & $\Omega(n/\log n)$ \\
\hline
\end{tabular}
}
\bigskip
\end{table}

\bigskip
\begin{tabular}{c|c}

\end{tabular}

An $st$-connectivity function associated with a graph $G$ can be represented by a read-once formula if and only if the graph $G$ is series-parallel~\cite{RaghavanSchach90}.
Thus our lower bound on the adaptivity gap for read-once formulas also applies to the problem of $st$-connectivity in uncertain networks.  \lisa{say something about Fu et al.'s experimental adaptivity gap observations?}

\bigskip
All of our lower bounds apply even to the case of unit costs $c_i=1$. These non-constant gaps contrast 
with the constant-factor adaptivity gaps shown previously for
the SBFE problem for symmetric functions and for linear threshold functions~\cite{gkenosisetal18}.
%
%
%.  Grammel et al.\ showed an upper bound of 4 on the additivity gap for the class of symmetric functions in the unit-cost case (and smaller gaps for certain subclasses of the symmetric functions)~\cite{}. Ghuge et al.\ showed an upper bound of $8+\epsilon$, on the adaptivity gap for the class of symmetric functions and the class of linear threshold functions, under arbitrary costs~\cite{}.  


 \lnf{shall we also mention the constant adaptivity gap for many other stochastic discrete optimization problems? e.g. stochastic knapsack, probing, covering, etc.}\lisa{I think it's enough to contrast with the previous SBFE results, especially now that I've been able to add the recent Ghuge et al. results.}

Our result for read-once formulas has implications for a problem of determining $st$-connectivity in an uncertain network, studied by Fu et al.~\cite{DBLP:journals/ton/FuFXPWL17}.  Consider a network (multi-graph) with designated nodes $s$ and $t$.  Suppose each edge $e$ in the network has an associated probability $p_e$, which is the probability that the edge is usable. This probability is independent of the probability that other edges are usable.
The $p_e$ values are given, and we need to determine whether or not there is a path of intact edges from $s$ to $t$.  Testing the usability of edge $e$ incurs a given cost $c_e$.  The problem is to determine the order in which to test the edges so as to minimize expected testing cost.  This is actually an SBFE problem, with the $x_i$ corresponding to the edges in the graph. \lnf{Would it be helpful to say, the $st$-connectivity problem in an uncertain network corresponds to the SBFE problem for DNF? As each possible s-t path is a term, and each edge on that path is a variable in that term}\lisa{Every Boolean fn can be represented by a DNF.  Because we define $f$ here, it immediately follows that there is a DNF associated with $f$.  So every SBFE problem is an SBFE problem for DNF -- sort of.  I say sort of because if we're concerned about computational complexity, then we need to take into account how the Boolean function is represented, which determines the size of the input. But in this paper, we do not worry about computational complexity. }  Here $f(x_1, \ldots, x_n)$ is a Boolean function such that $f(x)=1$ if and only if there exists an s-t path in the multi-graph such that for each edge in the path, we have $x_i=1$ for the corresponding $x_i$.  The multi-graph is two-terminal series-parallel, with terminals $s$ and $t$, if and only if the function $f$ is representable by a read-once formula~\cite{RaghavanSchach90}.  (We define series-parallel graphs in Section~\ref{preliminaries}.)
Thus the lower bound on the adaptivity gap for read-once formulas is also a lower bound on the adaptivity gap for the $st$-connectivity problem.  

We note that, as originally shown by Deshpande et al.\cite{DeshpandeGoalValue}, one approach to solving SBFE problems is to reduce them to special cases of Stochastic Submodular Cover.  As shown by~\cite{DBLP:conf/soda/AgarwalAK19}, the adaptivity gap for the general Stochastic Submodular Cover problem is linear in $n$ DOUBLE-CHECK THIS.  However, their result does not imply lower bounds on the adaptivity gap for SBFE problems.  

At the end of this paper, we perform experiments comparing the performance of optimal adaptive strategies and optimal non-adaptive strategies on $st$-connectivity problems, building on previous experiments of Fu et al~\cite{DBLP:journals/ton/FuFXPWL17}.
To compute optimal adaptive strategies, we use an exponential-time dynamic programming approach which has been rediscovered by a number of different researchers, including by Fu et al.~\cite{DBLP:journals/ton/FuFXPWL17} (see also \cite{}).\lisa{Mentioned in Unyulurt survey as having been used for linear threshold function, the data mining paper on optimal decision trees, also the Raghavan and ?? paper, also Fu et al.}  To compute optimal non-adaptive strategies, we develop a new dynamic programming algorithm, also taking exponential time.  This algorithm can be used to generate the optimal non-adaptive strategy solving the SBFE problem for any Boolean function.  

%Because of the exponential running time of the dynamic programming algorithms, we only run these algorithms on small datasets.  To explore the benefit of adaptivity on arger datasets, we compare the performance of existing and/or simple adaptive and non-adaptive heuristics.  
%Our experiments expand on previous experiments of
%Fu et al.\, who investigated different heuristics for solving the $st$-connectivity problem, some adaptive and some non-adaptive.

\subsection{Preliminaries}\label{preliminaries}
Consider a Boolean function $f:\{0,1\}^n \rightarrow \R$
and a strategy $S$ for testing variables on an unknown
input $x \in \{0,1\}^n$ to determine $f(x)$.
Define $\cost(f, x, S)$ to be the cost of determining
$f(x)$ using strategy $S$.
Then let $\cost(f, S)$ be the expected
cost of evaluating $f(x)$ where $x$ is drawn
from the uniform distribution, i.e.,
$$\cost(f, S):= \E_{x \sim \{0,1\}^n}[\cost(f,x,S)].$$
Let $\A$ denote the set of all adaptive
strategies for evaluating $f$ on an input
and let $\N$ denote the set of all
non-adaptive strategies for evaluating $f$.
Then 
$$\cost_\A(f):= \min_{S \in \A} \cost(f, S)
\textnormal{ and }
\cost_\N(f):= \min_{S \in \N} \cost(f, S).$$
With this notation in hand,
the adaptivity gap of a function $f$ is 
$\cost_\N(f)/\cost_\A(f)$.

A {\em read-once (Boolean) formula} is a tree, each of whose internal nodes is labeled either $\vee$ or $\wedge$. The internal nodes  have 2 or more children. 
Each leaf is labeled with a Boolean variable $x_i \in \{x_1, \ldots, x_n\}$.  The formula computes a Boolean function in the usual way.\footnote{Some definitions of a read-once formula allow negations in the internal nodes of the formula.  By DeMorgan's laws, these negations can be ``pushed'' into the leaves of the formula,
resulting in a formula whose internal nodes are $\vee$ and $\wedge$, such that each variable $x_i$ appears in at most one leaf, possibly with negation.}

A {\em DNF formula} is a Boolean formula of the form $T_1 \vee T_2 \vee \ldots T_k$ for some $k \geq 1$, such that each $T_i$ is the conjunction ($\wedge$) of literals.  A literal is a variable $x_i$ or a negated variable $\neg x_i$.  The $T_i$ are called the {\em terms} of the DNF formula.   The DNF formula is read-once if distinct terms contain disjoint sets of variables, without negations.

A two-terminal series-parallel graph (TTSP) is a graph which includes two distinct, distinguished nodes $s$ and $t$ (called terminal nodes). It is defined recursively as follows. An edge is a TTSP, with endpoints $s$ and $t$.  A multi-graph $G$ with terminal nodes $s$ and $t$ is a TTSP if it is produced by combining two TTSPs, $G_1$ and $G_2$, either in series, or in parallel, as follows.  
Let $s_1$, $t_1$ and $s_2$, $t_2$, be the two terminal nodes of $G_1$ and $G_2$, respectively.
\begin{itemize}
    \item Parallel: $G$ is  produced by merging nodes $s_1$ and $s_2$ into the single node $s$, and  merging nodes $t_1$ and $t_2$ into the single node $t$.  (If this results in multiple copies of the same edge, all copies are preserved.)
    \item Series: $G$ is  produced by merging nodes $t_1$ and $s_1$ into a new single node, and by setting $s = s_1$ and $t=t_2$.
\end{itemize}
By ``merging nodes $v$ and $w$ into the single node $z$'' we mean that whenever $v$ or $w$ appears as an endpoint of an edge, it is replaced by $z$.  
If this results in the creation of identical edges, all copies are preserved, so that the total number of edges remains the same after the merge.  
Given a multi-graph $G=(V,E)$ with two distinct distinguished nodes $s$ and $t$, define the {\em $st$-connectivity function} $f:\{0,1\}^E \rightarrow \{0,1\}$ of the graph as follows.  Function $f$ is a Boolean function whose variables correspond to the edges of $G$. For any assignment $a \in \{0,1\}^E$, $f(a)=1$ if and only if there is an $s-t$ path in $G$ such that all edges in the path are set to 1 by $a$.  
A Boolean function $f$ is expressible by a read-once formula if and only if it is the $st$-connectivity function of a two-terminal series-parallel graph~\cite{RaghavanSchach90}.
\footnote{
Some authors use the term ``series-parallel'' more narrowly, to refer to a graph produced by combining parallel networks in series (see, e.g.,~\cite{kowshik2011information}).  The $st$-connectivity functions of these graphs correspond to read-once CNF formulas.} 

\subsection{Literature Review}

\href{https://people.cs.rutgers.edu/~sa1497/stuff/papers/stochastic_submodular-cover_2019.pdf}{Stochastic Submodular Cover with Limited Adaptivity}

\href{https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8057094}{Complexity vs. Optimality: Unraveling
Source-Destination Connection in Uncertain Graphs}

\begin{itemize}
\item Read-Once DNF with Unit Costs and Uniform Probability:
$\Omega(\log n)$ lower bound and $O(\log n)$
\item Read-Once DNF with Unit Cost and Arbitrary Probability:
$\Omega(\sqrt{n})$ lower bound and $O(\sqrt{n})$
upper bound if constant length
\item Read-Once DNF with Arbitrary Cost and 
Uniform Probability: $\Omega(n^{1-\epsilon}/\log n)$
\item Read-Once Formula with Unit Cost and Constant Probability: $\Omega(\epsilon^3 n^{1-2\epsilon/\ln(2)})$ lower bound
\item DNF with Unit Costs and Uniform Probability:
$\Omega(n/\log n)$ lower bound
\end{itemize}

